RPS: Portfolio Asset Selection using Graph based Representation Learning

Portfolio optimization is one of the essential fields of focus in finance. There has been an increasing demand for novel computational methods in this area to compute portfolios with better returns and lower risks in recent years. We present a novel computational method called Representation Portfolio Selection (RPS) by redefining the distance matrix of financial assets using Representation Learning and Clustering algorithms for portfolio selection to increase diversification. RPS proposes a heuristic for getting closer to the optimal subset of assets. Using empirical results in this paper, we demonstrate that widely used portfolio optimization algorithms, such as MVO, CLA, and HRP, can benefit from our asset subset selection.

==> include/Conclusion.tex <==
\section{Conclusion}

This paper aimed to provide a new portfolio selection method that could outperform other algorithms used in the portfolio asset selection phase. To fulfill our goals, we provided a novel portfolio selection method based on representation learning and graph embedding called RPS. As seen in the results, various portfolio weight optimization methods can benefit from using RPS, since in every instance, using RPS selection improved the overall performance of the method versus the vanilla usage of that method. We have also seen that the portfolios constructed by RPS have a generally higher return than their rivals. Future directions can add dynamics to the problem and consider changing portfolios in time by periodic training RPS. Other weight optimization methods can also be tested on the selection to improve the portolios' performance further.

==> include/Evaluation.tex <==
\section{Evaluation Benchmark}

\paragraph{Minimum Spanning Tree (MST) and Hierarchical Clustering} The approach described in \cite{mantegna99paper} uses Kruskal's algorithm to build an MST over the complete graph of the market. The edges' weights are determined by the relation below.

\begin{equation}
d_{ij} = \sqrt{2(1 - \rho_{ij})}
\end{equation} 

where $\rho_{ij}$ is the correlation between asset $i$ and asset $j$. This approach relaxes the market graph and makes it easier for further operations. The paper itself does not specify a way to reach subsets of assets. We use Louvain Clustering Algorithm \cite{Blondel_2008} to extract smaller subsets of the market for evaluation. The clusters can be given to a weighting method, similar to RPS.

\paragraph{Graph Splex} The Graph Splex \cite{splex} tries to reach a diversified portfolio by creating a clique-like substructure of the market assets. We implemented this method using the pseudo-code described in the body of \cite{splex}. This subdivision can be weighted using the weight methods.

\paragraph{Simulated Annealing} Overall, various hill-climbing algorithms can be used as the solution for portfolio optimization cardinality problems, such as Simulated Annealing and Genetic Algorithms. The method starts with a random set of states for a subset of assets and changes the weights until a stable state is reached \cite{crama-schyns03, maringer05}.

\paragraph{Random Subsets} Since our goal is to constraint the cardinality of assets, we can use random divisions of the market as a baseline method. In this approach, Since random subdivision has access to every market subset, there is a probability that it can reach some of the best baskets. After selecting this subdivision, we can run the optimization methods on the portfolios.

==> include/FutureWorks.tex <==
\section{Future works}
% \begin{itemize}
%     \item Perioding?
%     \item Dynamic of portfolio
%     \item Preferences?
%     \item Other datasets (like tweets)
%     \item Graph representation with supervision or other data
% \end{itemize}
Our proposed model finds portfolio weights based on a fixed training period and suggest buying stock shares for the next period. One future direction would be to alter the model to offer buy/sell signals in real-time to achieve a more actionable model. This way, we could also consider other trading constraints and complexities like trade limits and trading costs. Additionally, our model just uses price time series to find relationship between different shares. We could also leverage news articles or related tweets sentiments as another source of information. Finally, the graph representation learning module used in this work is an unsupervised learning method that finds underlying relations between shares. Using supervisionfrom the next periods, we could enable the model to learn price dynamics and consider these dynamics in finding share similarities that are optimized for future periods.

==> include/Introduction-2.tex <==
For decades, Portfolio construction and optimization have had investors' attention. Financial institutions have long been pursuing methods to increase their returns further while also controlling their risks.

In this paper, we try to address this matter by proposing a two-phased portfolio construction method. This method first selects a subset of assets and then weights the obtained assets. While many portfolio optimization methods do not select the assets explicitly before weighing them, we focus on portfolio selection in this paper. We will indicate that we will reach better portfolios with higher returns and less risk by separating the portfolio asset selection phase from the portfolio weighting phase. Furthermore, we state that doing so would help us to overcome multiple issues. Firstly, it eliminates the covariance estimation inaccuracy which exists in previous portfolio optimization methods. Secondly, it resolves portfolio optimization algorithms such as MVO, which would have convergence problems if given an extensive benchmark of assets by pre-selecting a heuristically optimal subset of assets.

On its own, Portfolio construction is a classic research field in the finance area. However, with the growing influence of computational and machine learning methods, it can perhaps be seen from another perspective as an intermediary field. With that in mind, creative computational methods for this classic problem will start to rise. We are presenting in this paper is a novel method for stock selection using representation learning methods.
For portfolio selection and, more generally, portfolio construction, asset similarity plays a substantial role. Experts measure the similarity between assets in different ways, namely correlation, covariance, and granger causality (See, e.g.,   \cite{akhtaruzzaman2020influence,berger2020short,apergis2021cyclicality}). Whatever the measurement for the similarity may be, the ultimate goal is to reach diversification in portfolios by selecting uncorrelated assets for them.


In this paper, we redefine the similarity measurement of pairwise assets by defining a new distance for assets based on their correlation matrix by using Node2Vec. Moreover, with these sets of distances in our new embedding space, an uncorrelated set of assets can be selected using clustering methods. This procedure gives us a subset of assets that we can assign weights to the selected assets using a portfolio optimization algorithm. 

This paper will provide portfolio optimization algorithms a subset of assets using our portfolio selection method, which we will call RPS (Representation Portfolio Selection), and we will show that using our subset asset selection method, a portfolio optimization method's performance can be enhanced.  We applied RPS to widely used portfolio optimization algorithms such as CLA, HERC, HRP, and MVO, and for each of them, we observed that RPS improved their performance.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=\textwidth]{main/images/method diagram.png}
    \caption{Stages of RPS algorithm.}
    \label{fig:methoddiagram}
\end{figure*}

\input{main/include/RelatedWorks-2}

==> include/Introduction-3.tex <==
For decades, Portfolio construction and optimization have had investors’ attention. Financial institutions have long been pursuing methods to increase their returns further while also controlling their risks. The main goal in Portfolio Construction is to select a set of assets from a variety of  asset classes, and allocate investment weights to them, with the objective to maximise the overall investment return based on the given investment strategy and risk profile. The rather holistic approach of Portfolio Construction, aims to create a consistent flow of return in the long term, and to protect the investor from the market downturns, thus making Portfolio Construction methodologies valuable to numerous financial institutions and investors.

Over the course of time, lots of different techniques and approaches formed to address the issue of portfolio optimization. One of the first and most famous theories was Markowitz’s Portfolio Theory [cite, 1952]. In his study, he utilized the covariance matrix of the financial assets to define the problem as a quadratic programming problem. The success of Markowitz’s theory embarked on the creation of many other methods in this field, and in fact most of portfolio construction and optimization methods have used the core idea of Markowitz’s theory, which is tha the lower the correlation of a portfolio's assets, the lower the risk of that portfolio. To point out a few successful portfolio construction methods based on Markowitz modern portfolio theory, we can name CLA [2013, cite] and MVO [cite]. There are also some other well-known approaches that are based on computational algorithms such as clustering, including HRP [cite], HERC [cite], and NCO [cite].

Moreover, a body of literature investigates the portfolio selection method, which is to select a subset of assets that are a good choice set for portfolio construction. This was done both by using network methods like finding spanning trees on correlation-based graphs \cite{mantegna1999hierarchical} \cite{tumminello2010correlation} and other clustering methods like k-means and hierarchical clustering \cite{lemieux2014clustering} \cite{raffinot2017hierarchical} \cite{leon2017clustering}.

While portfolio construction is a classic research field in the finance area, with the growing influence of computational and machine learning methods, it can be seen from another perspective as an intermediary field. With that in mind, creative computational methods for this classic problem will start to rise. Some methods first predict each asset changes in the future and use the results for portfolio construction \cite{ta2018prediction}, \cite{chen2021mean}  \cite{ma2021portfolio}. Other methods have been also used to directly construct the portfolios by training on previous data, such as Reinforcement Learning \cite{yu2019model}, and Deep Learning \cite{2005.13665}. A core characteristic of the asset markets, in general, is the complexity of them. Having a robust way to deal with this complexity will be useful to solve the portfolio optimization problem. One of the machine learning methods that can be used to do so is Representation learning, which is a learning method that embeds the entities in the problem in a low-dimensional feature space. For instance, \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method is able to identify groups of stocks that had similar price behavior as well as similar news. On the other hand, \cite{hu2018deep} uses candlestick images and image neural network architectures to reach a proper representation for each stock.

In this paper, we try to address this matter by using a representation method on asset similarity graphs, which we construct using the correlation matrix of assets. We leverage these representations in a two-phased portfolio optimization setting. We select a subset of assets first and then weight the obtained assets. While many portfolio optimization methods do not select the assets explicitly before weighing them, we focus on portfolio selection in this paper. We will indicate that we will reach better portfolios with higher returns and less risk by separating the portfolio asset selection phase from the portfolio weighting phase. Furthermore, we state that doing so would help us to overcome multiple issues. Firstly, it eliminates the covariance estimation inaccuracy which exists in previous portfolio optimization methods. Secondly, it resolves portfolio optimization algorithms such as MVO, which would have convergence problems if given an extensive benchmark of assets by pre-selecting a heuristically optimal subset of assets.

% There are variety of machine learning methods used for constructing portfolios. Some methods leverage optimization methods to overcome computational and estimation problems of portfolio optimization methods. \cite{still2010regularizing} uses a regularization method to construct weights that are stable and robust to fluctuations. \cite{perrin2020machine} investigates optimization methods to find a method that could be practically used for real-world problems with lots of assets. Some other studies, use prediction models to first predict each assets future dynamics and then use the predictions to find optimal assets. \cite{ta2018prediction}, \cite{chen2021mean}, \cite{ma2021portfolio} investigate a range of machine learning methods from simpler methods (Linear Regression \& Support Vector Regression) to more complex methods (XGBoost \& LSTMs). RL methods have also been studied, in which an agent learns how to construct appropriate portfolios by behaving in the environment \cite{yu2019model}.

% Moreover, representation learning methods have also been studied for portoflio optimization recently. For instance, \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method is able to identify groups of stocks that had similar price behavior as well as similar news. On the other hand, \cite{hu2018deep} uses candlestick images and image neural network architectures to reach a proper representation for each stock.


%We design the method is a way that the distance measure in the embedding space would represent how much the two assets are correlated.

% 

% In this paper, we try to address this matter by using a representation method on asset similarity graph. We leverage these representations in a two-phased portfolio optimization setting. We select a subset of assets first and then weight the obtained assets. While many portfolio optimization methods do not select the assets explicitly before weighing them, we focus on portfolio selection in this paper. We will indicate that we will reach better portfolios with higher returns and less risk by separating the portfolio asset selection phase from the portfolio weighting phase. Furthermore, we state that doing so would help us to overcome multiple issues. Firstly, it eliminates the covariance estimation inaccuracy which exists in previous portfolio optimization methods. Secondly, it resolves portfolio optimization algorithms such as MVO, which would have convergence problems if given an extensive benchmark of assets by pre-selecting a heuristically optimal subset of assets.

% For portfolio selection and, more generally, portfolio construction, asset similarity plays a substantial role. Experts measure the similarity between assets in different ways, namely correlation, covariance, and granger causality (See, e.g.,   \cite{akhtaruzzaman2020influence,berger2020short,apergis2021cyclicality}). Whatever the measurement for the similarity may be, the ultimate goal is to reach diversification in portfolios by selecting uncorrelated assets for them.

% In this paper, we redefine the similarity measurement of pairwise assets by defining a new distance for assets based on their correlation matrix by using Node2Vec. Moreover, with these sets of distances in our new embedding space, an uncorrelated set of assets can be selected using clustering methods. This procedure gives us a subset of assets that we can assign weights to the selected assets using a portfolio optimization algorithm. 

% This paper will provide portfolio optimization algorithms a subset of assets using our portfolio selection method, which we will call RPS (Representation Portfolio Selection), and we will show that using our subset asset selection method, a portfolio optimization method's performance can be enhanced.  We applied RPS to widely used portfolio optimization algorithms such as CLA, HERC, HRP, and MVO, and for each of them, we observed that RPS improved their performance.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=\textwidth]{main/images/method diagram.png}
    \caption{Stages of RPS algorithm.}
    \label{fig:methoddiagram}
\end{figure*}

\input{main/include/RelatedWorks-3}

==> include/Introduction-4.tex <==
\section{Introduction}
Deciding how and where to invest money is one of the main challenges anyone with some savings faces. The complexity of finding an answer to this challenge has increased as the options for investment have grown in time, from gold and land to a myriad of financial assets like stocks, currencies, and cryptocurrencies. Moreover, investing money will be more important when the amount of money is considerable, such as for financial institutes, where any wrong decision or any fluctuation in the price of the invested asset can lead to considerable losses. In this situation, each individual can decide how to invest their money based on different parameters like knowledge, beliefs, and future predictions.

Two crucial concepts help investors diversify their assets. First is constructing an initial portfolio, which is a collection of financial assets that one individual holds. The second is managing the portfolio afterward. While these two concepts are interlinked, the dynamics of assets and trading constraints in markets introduce more complexities than the former, making them two different problems to solve. This paper will focus on the first problem, portfolio construction, and leave analyzing the complexities of portfolio management to future studies. Studies on the portfolio optimization problem have a long history. One of the first and most famous theories that studied portfolio construction was Markowitz's Portfolio Theory \cite{markowitz52, markowitz59, markowitz87}, which became the cornerstone of modern portfolio theory. In his study, he utilized the covariance matrix of the financial assets to define the problem as a quadratic programming problem. The success of Markowitz's theory embarked on creating many other methods in this field with different ideas. However, most portfolio construction and optimization methods have used the core idea of Markowitz's theory: the lower the correlation of a portfolio's assets, the lower the risk. Although naturally, many papers started studying the shortcomings of Markowitz's methods and addressed solutions to those shortcomings \cite{eltongruber95, king93, konnoyamazaki91, milis97, mitra2003review, rockafellar2000optimization}.

One of the Markowitz issues that we mitigate in this paper is the cardinality constraint problem. Markowitz’s method outputs the fraction of money to invest on each asset, with the assets and price history as the input. There are thousands of various assets available for investment, which can lead to hardships since managing such portfolios can be complicated. Moreover, it can be shown that limiting assets to a maximum count is a form of the Knapsack problem, which is computationally NP-hard \cite{garey-johnson79}. Different methods use different types of heuristics to solve this issue. For example, Crama and Schyns \cite{crama-schyns03} and Maringer \cite{maringer05} used simulated annealing, while others use clustering methods like k-means and hierarchical clustering \cite{lemieux2014clustering, raffinot2017hierarchical, leon2017clustering}. A whole family of other solutions formed based on Mantegna’s Minimum Spanning Tree method \cite{mantegna99book, mantegna99paper}. Some other methods try to reformulate the problem and solve it mathematically, such as Cesarone et al. \cite{Cesarone2013ANM}.

With the growing influence of computational and machine learning methods on financial markets, portfolio construction can be seen as an intermediary field from another perspective. A variety of computational methods have started to rise. Some methods first predict each asset changes in the future and use the results for portfolio construction \cite{ta2018prediction, chen2021mean, ma2021portfolio}. Other methods have also been used to directly construct the portfolios by training on previous data, such as Reinforcement Learning \cite{yu2019model}, and Deep Learning \cite{zhang2020deep}. A core characteristic of the asset markets, in general, is their complexity. Having a robust way to deal with this complexity will be useful to solve the portfolio optimization problem. One of the machine learning-based methods that can be used to do so is Representation learning, which is a learning method that embeds the entities in the problem in a low-dimensional feature space. For instance, \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method can identify groups of stocks that had similar price behavior as well as similar news. On the other hand, \cite{hu2018deep} uses candlestick images and image neural network architectures to obtain a proper representation for each stock.

A new family of representation learning methods has formed in recent years, which embed the nodes of the graphs using their connections. This paper addresses the portfolio construction problem using the Node2Vec \cite{grover2016node2vec} method, a graph representation learning algorithm, on asset similarity graphs using the correlation matrix of assets. We leverage these representations in a two-phased portfolio optimization setting. First, we select a subset of assets and then weigh the obtained assets. While many portfolio optimization methods do not select the assets explicitly before weighing them, we focus on portfolio selection in this paper. We will indicate that better portfolios with higher returns and less risk can be achieved by separating the portfolio asset selection phase from the portfolio weighting phase. Furthermore, we state that doing so would help us to overcome multiple issues. Firstly, it eliminates the covariance estimation inaccuracy which exists in previous portfolio optimization methods. Secondly, it resolves portfolio optimization algorithms such as Mean-Variance Optimization (MVO) \cite{erlich2010MVO}, which would have convergence problems if given an extensive benchmark of assets by pre-selecting a heuristically optimal subset of assets.

 The paper is organized in the following structure.  Section II provides an in-depth description of the proposed method.  Section III discusses the other baseline methods that can be used for the portfolio selection problem.  At last, the results of the evaluation on multiple datasets are provided in section IV.


==> include/Introduction.tex <==
\section{Introduction}
% \begin{itemize}
%     \item What is the portfolio optimization problem?
%     \item What are the already available solutions?
%     \item Previous works problems.
%     \item What is our proposed solution?
%     \item Why is our method, good?
%     \item Structure of the paper.
% \end{itemize}
For decades, Portfolio construction and optimization has had the attention of investors, financial institutions have long been pursuing methods to further increase their returns, while also controlling their risks. 
Portfolio construction has two main key parts, the first part is asset selection, and the second part is weighting the assets held in the portfolio. Weighting a given benchmark of assets implicitly also includes Portfolio selection. In other words, many portfolio optimization methods do not select the assets explicitly before weighting them. In this paper, we separate these two parts and focus on the portfolio selection process, and indicate that pre-selection of benchmark and weighting the selected subset of assets afterward reaches better results.
On its own, Portfolio construction is a classic financial research area, but with the growing influence of computational methods and machine learning over other fields, it can perhaps be seen from another perspective, as an intermediary field, and with that in mind, creative computational methods for this classic problem will start to rise. That is what we are presenting in this paper, a novel method for stock selection using representation learning.
For portfolio selection and more generally, portfolio construction, asset similarity plays a substantial role. The similarity between assets can be and has been measured in different ways, namely correlation, Covariance, and Granger causality [reference papers]. Different approaches have been taken before, but whatever the measurement for the similarity may be, the ultimate goal is to reach diversification in our portfolio by selecting uncorrelated assets for the portfolio.
In this paper, we redefine the similarity measurement of pairwise assets by defining a new distance for each pair of assets based on their correlation matrix, by using Node2Vec. And with these sets of distances in our new embedding space, an uncorrelated set of assets can be selected by using clustering methods. This gives us a subset of assets that we can assign weights to the selected assets using a portfolio optimization algorithm. 
In this paper, we will provide portfolio optimization algorithms a subset of assets using our portfolio selection method, which we will call RPS (Representation Portfolio Selection), and we will show that using our subset asset selection method, a portfolio optimization method's performance can be enhanced.  We applied RPS to widely used portfolio optimization algorithms such as CLA, HERC, HRP, and MVO, and for each of them, we observed that RPS improved their performance.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.8\textwidth]{templates (1)/images/method diagram.png}
    \caption{Stages of RPS algorithm.}
    \label{fig:methoddiagram}
\end{figure*}

\input{templates (1)/include/RelatedWorks}

==> include/Method-2.tex <==
\section{Method}

This paper aims to present a novel utilization of representation learning as a diversification heuristic for a portfolio. The main idea is to choose uncorrelated assets for a portfolio to minimize the portfolio variance, which means less risk for the portfolio.
To elaborate, take $N$ assets in a portfolio which are pairwise uncorrelated, i.e., $\forall i \neq j, \rho_{i j}=0 .$ Then the variance for this portfolio would be 

$$
Var\left(P\right)=\sum_{i=1}^{N}\left(w_{i}\right)^{2} \sigma_{i}^{2}
$$


And to better show the idea, with the simplifying assumption of equal weights for the assets, i.e., $i, w_{i}=1 / N,$ we will have

$$
Var\left(P\right)=\frac{1}{N^{2}} \sum_{i=1}^{N} \sigma_{i}^{2} \leq \frac{\sigma_{M}^{2}}{N}
$$
where $$ \sigma_{M}=\max \left[\sigma_{i}: i=1, \ldots, N\right]$$

And as $N$ grows to infinity, $Var\left(P\right)$ will lean towards $0$. This shows us that the more pairwise uncorrelated assets we have in our portfolio, the smaller the portfolio's risk will be. Even though we do not have completely uncorrelated assets in real life, we can still build upon the shown idea and choose rather uncorrelated assets to reach a well-diversified low-risk portfolio. In this paper, we would want to build an augmented graph with some properties out of these assets based on their similarity or, to be more exact, their pairwise correlation, and then by applying a representation learning method on the graph, reach a new distance representation for the assets, which we can then choose the uncorrelated assets from to fulfill the idea shown above. 


To use machine learning and deep learning methods on graph-structured data, we must first embed the graph or its nodes in a vector space. There are different types of methods being used for this purpose. Some of them use discrete metrics to define the similarity between nodes like the number of common neighbors \cite{ahmed2013distributed, cao2015grarep}. Others use random walks, and the probability of observing one node while starting from another node as the similarity of the two nodes \cite{perozzi2014deepwalk, grover2016node2vec}. These two methods are unsupervised and do not require any labels on data. However, if we have some labeled data, we can employ other methods that utilize the labels to find better representations. These methods have been improved by using other properties of graphs \cite{kipf2016semi, hamilton2017inductive}. Since our data is unlabeled and our initial metric (correlation) was not discrete, we chose to use Node2Vec and apply it on the correlation graph of the stocks that we constructed to reach a new similarity metric so that ultimately we can select a set of stocks which gives us a diversified portfolio.

To build the described graph, we first need to set weights for the edges. We chose Pearson correlation as the basis of the pairwise similarity measure for the assets, and then we had to adjust the measurement for better results. As for the adjustment and why it is needed since we will be applying Node2Vec to the graph and as it is a random walk based algorithm on the weights of our graph, at a given node, it will iterate through the edge $j $ with a probability of $ \frac{w_{j}}{\sum_{i=1}^{n} w_{i}}$. So we have to augment the basic Pearson Correlation such that the more correlated the two assets are, the less the weight of their intermediate edge will be and vice versa. After applying Node2Vec, starting a random walk on a node, results in more visits to uncorrelated assets. Furthermore, to ensure that we will not be visiting high correlated assets for a starting node in a Node2Vec with a walk length of greater than 1, we should also consider these properties in our transformation function:

\begin{itemize}
    \item 
    As the corresponding correlation of an edge approaches 0, the edge's weight should approach infinity.
    \item
    As the corresponding correlation of an edge approaches 1, the edge's weight should approach 0.
\end{itemize}

We used hyperbolic cotangent for our weight adjustment as it supported such properties. Then, The new redefinition of pairwise similarity between assets which was also used as the weight of the edges in our graph is calculated this way:

\begin{equation}
w_{ij} = \mid \coth(Correlation(i,j)) \mid -\coth(1)
\end{equation}

\begin{figure}[]
    \centering
    \includegraphics[width=0.5\textwidth]{main/images/method_diagram.png}
    \caption{Stages of RPS algorithm.}
    \label{fig:methoddiagram}
\end{figure}

As our graph is built, the next step is to run Node2Vec on our graph. For each node, multiple random walks are executed based on the weights of its edges. That is, in each step, the algorithm visits the neighbor $j$ of a starting node with a probability of $ \frac{w_{j}}{\sum_{i=1}^{n} w_{i}}$, where $w_j$ is the weight of the edge between the starting node and neighbor $j$, and the algorithm iterates over the graph in this manner $l$ times for each execution, where $l$ is the walk-length of the algorithm. In the end, a new pair-wise distance representation is created based on the nodes visited during the execution of the algorithm for each starting node. Since we built the graph so that the edges with corresponding uncorrelated nodes to have greater weight than correlated ones, we will visit uncorrelated nodes for each node after this algorithm.

After embedding the nodes of the graph, we are free to use different clustering algorithms to reach our final portfolios. We used two different clustering methods. The first one was the k-means clustering algorithm, and the second one was the fuzzy c-means algorithm, which allows each node to be present in more than one subset. Our initial belief was that this relaxation might allow the procedure to achieve better performance. Since our representation of the graph is produced so that the uncorrelated assets are closer to each other, we will reach clusters of relatively uncorrelated assets, which can be interpreted as selected assets for our diversified portfolio.

The last step in the method is to input the resulted portfolios into a portfolio optimization method to calculate the fraction of wealth to invest in each of them. In this paper, we made use of three different optimization methods: MVO \cite{erlich2010MVO}, Hierarchical Risk Parity (HRP) \cite{pfitzinger2019HRP}, and Critical Line Algorithm (CLA) \cite{niedermayer2010CLA}.

==> include/Method.tex <==
\section{Method}
Our goal in this paper is to present a novel utilization of representation learning as a diversification heuristic for a portfolio. The main idea is to choose uncorrelated assets for a portfolio so that we can minimize the portfolio variance which means less risk for the portfolio.
To elaborate, take $N$ assets in a portfolio which are pairwise uncorrelated, i.e., $\forall i \neq j, \rho_{i j}=0 .$ Then the variance for this portfolio would be 

$$\operatorname{Var}\left(P\right)=\sum_{i=1}^{N}\left(w_{i}\right)^{2} \sigma_{i}^{2}$$


And to better show the idea, with the simplifying assumption of equal weights for the assets, i.e., $i, w_{i}=1 / N,$ we will have

$$
\operatorname{Var}\left(P\right)=\frac{1}{N^{2}} \sum_{i=1}^{N} \sigma_{i}^{2} \leq \frac{\sigma_{M}^{2}}{N}
$$
where $$ \sigma_{M}=\max \left[\sigma_{i}: i=1, \ldots, N\right]$$

And as $N$ grows to infinity,  $\operatorname{Var}\left(P\right)$  will lean towards $0 .$ This shows us, that the more pairwise uncorrelated assets we have in our portfolio, the smaller the risk of the portfolio will be. Even though we do not have completely uncorrelated assets in real life, we can still build upon the shown idea and choose rather uncorrelated assets to reach a well diversified low risk portfolio. In this paper, we would want to build an augmented graph with some properties out of these assets based on their similarity or to be more exact, their pairwise correlation, and then by applying node2vec on the graph, reach a new distance representation for the assets, which we can then choose the uncorrelated assets from to fulfil the idea shown above. 


To build the described graph, we first need to set weights for the edges. For this task we first need a pairwise similarity measure for the assets and then we have to adjust the measurement for better results. We chose Pearson correlation for as the basis of the similarity measurement, as our data was internal and correlation is [\todo{give reasons for correlation}]. As for the adjustment and why it is needed, since we will be applying node2vec to the graph and as it is a random walk based algorithm on the weights of our graph, at a given node, it will iterate through the edge $j $ with a probability of $ \frac{w_{j}}{\sum_{i=1}^{n} w_{i}}$. So we have to augment the basic Pearson Correlation such that the more correlated the two assets are, the less the weight of their intermediate edge should be and vice versa. This way after applying node2vec, starting a random walk on a node, results in more visits to uncorrelated assets. Furthermore, to ensure that we won't be visiting high correlated assets for a starting node in a node2vec with a walk length of grater than 1, we should also consider these properties in our transformation function:
\begin{itemize}
    \item 
    As the corresponding correlation of an edge approaches to 0, the edge's weight should approach infinity.
    \item
    As the corresponding correlation of an edge approaches to 1, the edge's weight should approach 0.
\end{itemize}


We used Hyperbolic Sine for our weight adjustment as it supported such properties. Then, The new redefinition of pairwise similarity between assets which was also used as the weight of the edges in our graph is calculated this way:

\begin{equation}
w_{ij} = \mid \coth(Correlation(i,j)) \mid -\coth(1)
\end{equation} 
As our graph is built, the next step is to run node2vec on our graph, for each node multiple random walks are executed based on the weights of its edges, that is in each step, the algorithm visits the neighbour $j$ of a starting node with a probability of $ \frac{w_{j}}{\sum_{i=1}^{n} w_{i}}$, where $w_j$ is the weight of the edge between the starting node and neighbour $j$, and the algorithm iterates over the graph in this manner $l$ times for each execution, where $l$ is the walk-length of the algorithm. In the end, a new pair-wise distance representation is created based on the nodes that have been visited during the execution of the algorithm for each starting node. Since we built the graph in a way that the edges with their corresponding nodes being uncorrelated, have a greater weight, we will visit uncorrelated nodes for each node after this algorithm.

We will then use soft k-means clustering on the newly created representation of our graph, and since our representation of the graph is produced so that the uncorrelated assets are closer to each other, we will reach clusters of rather uncorrelated assets which can be interpreted as selected assets for our diversified portfolio.



==> include/RelatedWorks-2.tex <==
\subsection{Related works}

After the initial widespread success of Markowitz's technique, lots of other approaches emerged in this area to enhance portfolio construction by modifying elements of the Markowitz technique or utilizing different approaches. Some attempts tried to improve the covariance estimation mechanism. \cite{ledoit2004well}\cite{wong2003efficient} Using graphs to model interactions between stocks is another approach. Mantegna (1998) was one of the first works that used graphs to suggest a portfolio. By finding an MST of the weighted graph, the method could find the hierarchical structure between stocks. Moreover, other combinatorial optimization methods are used to identify portfolios, as in \cite{boginski2014network}, which finding relaxed cliques in the network helps to identify similar stocks.

Machine learning techniques have also found their way in financial studies. In \cite{de2016building} authors use a hierarchical clustering approach to cluster stocks based on distances of their corresponding rows in the covariance matrix. Also, \cite{kumari2019mean} uses a k-means clustering approach to identify stock groups with the same characteristics.

Due to recent advances in deep learning methods, methods that try to use deep embeddings for stocks are also developed. For instance, \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method is able to identify groups of stocks that had similar price behavior as well as similar news. On
the other hand, \cite{hu2018deep} uses candlestick images and image neural network architectures to reach a proper representation for each stock.

While these representation learning methods use text and image data, to the best of our knowledge, no previous method uses the graph of relationships between stocks to derive embeddings for stocks.



==> include/RelatedWorks-3.tex <==
\subsection{Related works}

% Over the course of time, lots of different techniques and approaches formed to address the issue of portfolio optimization. One of the first and most famous theories was Markowitz’s Portfolio Theory [cite, 1952]. In his study, he utilized the covariance matrix of the financial assets to define the problem as a quadratic programming problem. The success of Markowitz’s theory embarked on the creation of many other methods in this field, and in fact most of portfolio construction and optimization methods have used the core idea of Markowitz’s theory, which is tha the lower the correlation of a portfolio's assets, the lower the risk of that portfolio. To point out a few successful portfolio construction methods based on Markowitz modern portfolio theory, we can name CLA [2013, cite] and MVO [cite]. There are also some other well-known approaches that are based on computational algorithms such as clustering, including HRP [cite], HERC [cite], and NCO [cite]. MANTANGE?

% There are variety of machine learning methods used for constructing portfolios. Some methods leverage optimization methods to overcome computational and estimation problems of portfolio optimization methods. \cite{still2010regularizing} uses a regularization method to construct weights that are stable and robust to fluctuations. \cite{perrin2020machine} investigates optimization methods to find a method that could be practically used for real-world problems with lots of assets. Some other studies, use prediction models to first predict each assets future dynamics and then use the predictions to find optimal assets. \cite{ta2018prediction}, \cite{chen2021mean}, \cite{ma2021portfolio} investigate a range of machine learning methods from simpler methods (Linear Regression \& Support Vector Regression) to more complex methods (XGBoost \& LSTMs). RL methods have also been studied, in which an agent learns how to construct appropriate portfolios by behaving in the environment \cite{yu2019model}.

After the initial widespread success of Markowitz’s technique, lots of other approaches emerged in this area to enhance portfolio construction by modifying elements of the Markowitz technique or utilizing different strategies. Some attempts tried to improve the covariance estimation mechanism \cite{ledoit2004well, wong2003efficient, ledoit2004well}. Other methods have considered higher-order moments to capture the relationships between assets better \cite{maringer2009global, khan2020sustainable}.

Instead of improving portfolio optimization methods directly, some methods approached the problem by first selecting a subset of assets and then weighting them to construct the portfolio. Mantegna \cite{mantegna99paper} was one of the works that did so by using graphs to suggest a subset of assets. By finding an MST of the weighted graph, the method could find the hierarchical structure between stocks. Moreover, other combinatorial optimization methods on graphs are used to identify portfolios, as in Boginski et al. \cite{boginski2014network}, in which finding relaxed cliques in the network helps identify similar stocks. Clustering techniques have also found their way into financial studies. In De Prado \cite{de2016building}, authors use a hierarchical clustering approach to cluster stocks based on distances of their corresponding rows in the covariance matrix. Also, Kumari et al. \cite{kumari2019mean} uses a k-means clustering approach to identify stock groups with the same characteristics.


Recently, machine learning methods have found their ways in financial market studies \cite{henrique2019literature}. Portfolio optimization was not an exception for this trend. Some methods in this area leverage optimization methods to overcome computational and estimation problems of portfolio optimization methods. \cite{still2010regularizing} uses a regularization method to construct weights that are stable and robust to fluctuations. \cite{perrin2020machine} investigates optimization methods to find a method that could be practically used for real-world problems with lots of assets. Some other studies use prediction models first to predict each asset's future dynamics and then use the predictions to find optimal assets. \cite{ta2018prediction, chen2021mean, ma2021portfolio} investigate a range of machine learning methods from simpler methods (Linear Regression \& Support Vector Regression) to more complex methods (XGBoost \& LSTMs \footnote{Long Short-Term Memory}). Reinforcement Learning (RL) methods have also been studied, in which an agent learns how to construct appropriate portfolios by behaving in the environment \cite{yu2019model}.

Due to the recent advances in deep learning methods, methods that try to use deep embeddings for stocks are also developed. For instance, Du \& Tanaka-Ishii \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method can identify groups of stocks that had similar price behavior as well as similar news. On the other hand, Hu et al. \cite{hu2018deep} uses candlestick images and image neural network architectures to reach a proper representation for each stock.

While these representation learning methods use text and image data, to the best of our knowledge, no previous method uses the graph of relationships between stocks to derive embeddings for stocks.



==> include/RelatedWorks.tex <==
\subsection{Related works}
% \begin{itemize}
%     \item The survey on portfolio selection.
%     \item The most basic available solutions
%     \item HRP, CLA
%     \item Graph-based solutions with the MST approach
%     \item Representation learning on candle images
% \end{itemize}
While Markowitz’s technique for portfolio optimization was a breakthrough method in financial asset management, its shortcomings are also well studied. The original intuition was to use the covariance matrix as an estimate for the connection between portfolios, to help invest in a diverse set of stocks that are their future is uncorrelated. However, major problems with this is method are investigated: (i) studies have shown that these estimations may not be accurate\cite{green1992will}\cite{ledoit2003improved}, and for having an appropriate estimate, the length of the historical data should grow as the number of stocks in interest grows. This issue will cause that in most real setups, this length should be as long as 3-4 years that is a long period and could not represent the recent relationships between stocks. \cite{chamberlain1982arbitrage}\cite{de2016building} (ii) output investment fractions are not stable, i.e., with introducing a small amount of noise to the data, the result could vary significantly.

To address these issues, lots of different approaches emerged in this area. Some attempts tried to improve the covariance estimation mechanism. \cite{ledoit2004well}\cite{wong2003efficient} Using graphs to model interactions between stocks is another approach. Mantegna (1998) was one of the first works that used graphs to suggest a portfolio. By finding an MST of the weighted graph, the method could find the hierarchical structure between stocks. Moreover, other combinatorial optimization methods are used to identify portfolios, as in \cite{boginski2014network}, which finding relaxed cliques in the network helps to identify similar stocks.

Machine learning techniques have also found their way in financial studies. In \cite{de2016building} authors use a hierarchical clustering approach to cluster stocks based on distances of their corresponding rows in the covariance matrix. Also, \cite{kumari2019mean} uses a k-means clustering approach to identify stock groups with the same characteristics.

Due to recent advances in deep learning methods, methods that try to use deep embeddings for stocks are also developed. For instance, \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method is able to identify groups of stocks that had similar price behavior as well as similar news. On the other hand, \cite{hu2018deep} uses candlestick images and image neural network architectures to reach a proper representation for each stock. While these representation learning methods use text & image data, to the best of our knowledge, no previous method uses the graph of relationships between stocks to derive embeddings for stocks. To use machine learning and deep learning methods on graph structured data we have to first embed the graph or its nodes in a vector space. This task is well addressed in literature as representation learning for graphs which is to find an appropriate way to represent graph elements to best preserve the properties and relations of nodes that are required for solving the problem. There are different types of methods being used. Some of them use discrete metrics to define the similarity between nodes like the number of common neighbors \cite{ahmed2013distributed}\cite{cao2015grarep}. Others use random walks and the probability of observing one node while starting from another node as the similarity of the two nodes \cite{perozzi2014deepwalk}\cite{grover2016node2vec}. These two methods are unsupervised and don't require any labels on data. However, in case we have some labeled data we can use other methods that can use the labels in finding good representations. These methods also can better use other graph features. \cite{kipf2016semi}\cite{hamilton2017inductive}. Since our data is unlabeled and our initial metric (corrolation) was not discrete, we chose to use node2vec to apply it on the correlation graph of the stocks that we constructed, to reach a new similarity metric so that ultimately we can select a set of stocks which gives us a diversified portfolio.


==> include/Results.tex <==
\section{Results}
% \begin{itemize}
%     \item values of them?
%     \item K/N portfolio $->$ methods that construct small baskets, heuristics
%     \item S&P, NYSE, ...
%     \item Sharpe, risk, return.
%     \item Efficient frontier.

%     \item Discuss how changes in hyperparameters affect the results.
% \end{itemize}

% To evaluate the [RPS+optimization] model, we tested the results against various portfolio optimization algorithms. Since RPS is a portfolio selection algorithm, it can be combined with a generic type of optimization methods to enhance the performance of that particular algorithm. For this purpose, we used MVO[cite], CLA[cite], HRP\cite{de2016building}, and HERC[cite] to show RPS+optimization algorithm performs better than the algorithms themselves, without a selection method. These results show that a pre-selection of the portfolio is a dominant strategy to using the optimization algorithms alone, and furthermore, we show that our method performs better than other selection+optimization methods, such as random selection. [and simulated annealing?]
% For evaluating the created portfolios, we used efficient frontier and several financial criteria.
% [discussion]
% \begin{itemize}
% \item Sharpe Ratio:

% \begin{equation}
%     Sharpe\ Ratio = \frac{R_{p} - r_{f}}{\sigma_{p}}
% \end{equation}

% Where $R_{p}$ is return of the portfolio, $r_{f}$ is the risk free rate of return, and $\sigma{p}$ is the standard deviation of portfolio.

% \item Information Ratio:

% \begin{equation}
%  Information\ Ratio = \frac{R_{p} - R_{b}}{\sigma_{R_{p} - r_{b}}}     
% \end{equation}

% Where $R_{p}$ is return of the portfolio, $R_{b}$ is return of the benchmark, and $\sigma_{R_{p} - r_{b}}$ is the standard deviation of the excess return.

% \item
% M2 Measure (Modigliani):
% \begin{equation}
%  M2\ Measure = SR * \sigma_{b} + r_{f}   
% \end{equation}
% Where $SR$ is the Sharpe Ratio, $r_{f}$ is the risk free rate of return, and $\sigma_{b}$ is the standard deviation of benchmark.

% \end{itemize}
% [the above criteria are correlated somehow]

% To evaluate the [RPS+optimization] model, we have chosen the S&P dataset for training. We first trained the model on [folan] timeframe to attain the optimal selection. Then, we weighted the selections using the algorithms explained above and sorted the training results according to the criteria to achieve the best-selected portfolios. After this training phase, we used the exact weights to evaluate the portfolios in the next [timeframe].


% Also, table [number] shows the evaluation of methods using the mentioned criteria.

% [table]

% As it can be seen, we can enhance every optimization algorithm using pre-selection with the RPS model.

% RPS+OA vs. Random Pre-Selection+OA
% To show that the selected portfolios by the RPS method are solid selections, we evaluate the previous measurements for randomly selected portfolios. As a random portfolio has access to the whole efficient frontier area, a sufficient subset of random portfolios can sample the entire area, and thus, it would contain top portfolio selections.

% According to Figure \ref{fig:our_selection}, we can see that RPS+each optimization performs better than top random selections with the same optimization.


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{images/contribution-1-with-legend-all-dot.png}
    \caption{The efficient-frontier plot for the top 6 portfolios of the training set for RPS+optimization versus the algorithms without any selection phase.}
    \label{fig:our_selection}
\end{figure}

The data-set that we chose as a benchmark for our empirical results was S\&P 500, we used [timeframe] for training and [timeframe] as the testing period. Every weighted portfolio during the training period was evaluated with multiple financial ratios and the best performing portfolios were used in the following test timeframe.
The financial ratios which we used to evaluate the portfolios were as following:

\begin{itemize}
\item Sharpe Ratio:

\begin{equation}
    Sharpe\ Ratio = \frac{R_{p} - r_{f}}{\sigma_{p}}
\end{equation}

Where $R_{p}$ is return of the portfolio, $r_{f}$ is the risk free rate of return, and $\sigma{p}$ is the standard deviation of portfolio.

\item Information Ratio:

\begin{equation}
 Information\ Ratio = \frac{R_{p} - R_{b}}{\sigma_{R_{p} - r_{b}}}     
\end{equation}

Where $R_{p}$ is return of the portfolio, $R_{b}$ is return of the benchmark, and $\sigma_{R_{p} - r_{b}}$ is the standard deviation of the excess return.

\item
M2 Measure (Modigliani):
\begin{equation}
 M2\ Measure = SR * \sigma_{b} + r_{f}   
\end{equation}
Where $SR$ is the Sharpe Ratio, $r_{f}$ is the risk free rate of return, and $\sigma_{b}$ is the standard deviation of benchmark.

\end{itemize}

We have done two sets of experiments which we will present.

\begin{table*}[!h]
\centering
\caption{Portfolios built with different settings can be seen here with their respective performance measurements. It can be seen that for each different portfolio optimization algorithm, applying RPS as an asset selection method improves the performances for the portfolio.}
\label{tab:evaluations}
\begin{tabular}{l|c|c|c|}
\cline{2-4}
                                              & \multicolumn{1}{l|}{Sharpe Ratio} & \multicolumn{1}{l|}{Information Ratio} & \multicolumn{1}{l|}{Modiliani Risk Adjusted Performance} \\ \hline
\multicolumn{1}{|l|}{\textbf{RPS+MVO}}        & 5.785917                          & 4.151003                               & 1.345936                               \\ \hline
\multicolumn{1}{|l|}{Best Random Subset+MVO}  & 5.014807                          & 3.459654                               & 1.167744                               \\ \hline
\multicolumn{1}{|l|}{MVO}                     &            -                       &                                        &                                        \\ \hline
\multicolumn{1}{|l|}{\textbf{RPS+HRP}}        & 4.507241                          & 2.851294                               & 1.050454                               \\ \hline
\multicolumn{1}{|l|}{Best Random Subset+HRP}  & 3.607982                          & 3.826712                               & 0.842649                               \\ \hline
\multicolumn{1}{|l|}{HRP} &     -1.276275               &                                   &                                                                                \\ \hline
\multicolumn{1}{|l|}{\textbf{RPS+HERC}}       & 4.458710                          & 2.703551                               & 1.039239                               \\ \hline
\multicolumn{1}{|l|}{Best Random Subset+HERC} & 2.664600                          & 1.970464                               & 0.624648                               \\ \hline
\multicolumn{1}{|l|}{HERC}  &        -1.294033           &                                   &                                                                                \\ \hline
\multicolumn{1}{|l|}{\textbf{RPS+CLA}}        & 6.734292                          & 4.480901                               & 1.565091                               \\ \hline
\multicolumn{1}{|l|}{Best Random Subset+CLA}  & 8.920160                          & 4.928809                               & 2.070211                               \\ \hline
\multicolumn{1}{|l|}{CLA}    &    -1.924916             &                                   &                                                                                \\ \hline
\end{tabular}
\end{table*}

\subsection{RPS+POA vs. POA}

Since RPS is a portfolio selection algorithm, it can be combined with a generic type of Portfolio Optimization Method to enhance the performance of that algorithm. To evaluate the RPS method, we used selected subsets of assets calculated by RPS, and optimized the subsets with various optimization methods such as CLA[cite], HRP\cite{de2016building}, and HERC[cite], thus reaching a weighted portfolio which we will call RPS+POA (Representation Portfolio Selection + Portfolio Optimization Algorithm). Then we compared performance of the RPS+POA portfolio with the portfolio built with the corresponding Portfolio Optimization Algorithm, which is shown in Figure \ref{fig:our_selection}.
As it is indicated in the the figure, RPS enhances all of the mentioned portfolio optimization algorithms. The numerical comparisons are shown in Table \ref{tab:evaluations}.

Furthermore there are portfolio optimization algorithms which can not be used on a whole benchmark of assets and they need to have a subset of assets so that they can operate functionally. For instance, MVO[cite] might not converge when given a big benchmark of assets. Such methods benefit from the asset selection of RPS.

\subsection{RPS+POA vs. Random-Selected-Assets+POA}

To  show  that  the  selected  portfolios  by  the  RPS  method are  solid  selections,  we  evaluate  the  previous  measurements for  randomly  selected  portfolios.  As  a  random  portfolio  has access  to  the  whole  efficient  frontier  area,  a  sufficient  subset of  random  portfolios  can  sample  the  entire  area,  and  thus,  it would contain top portfolio selections. We generated more than 13k random portfolios, which took the same time as RPS to train on the market data and calculate its heuristically optimal subset of assets. Figure 3 shows the comparison between performance of RPS+POA portfolios and Random-Selected-Assets+POA portfolios on test data. Since only the top random portfolios of the train data will be chosen as potential portfolios for the test data, only the top 5(?) portfolios in terms of Sharpe Ratio out of all the generated Random-Selected-Assets have been shown on this figure.



% [explain the extra column, the betterness-average]
% [RPS+OA vs. other pre-selections?+OA]


%We chose S&P500 stocks for practical demonstration of our portfolio selection algorithm, we call our method RPS (Representation Portfolio Selection). To show how RPS and pre-selection of assets improves portfolio optimization methods, we built several portfolios using different portfolio optimization algorithms with 3 different variations, with no asset selection beforehand, with pre-selection using random assets, and with RPS asset selection method which we proposed in our papaer. The results can be seen in table 1, where it shows that that for each portfolio optimization method, the RPS variant outperforms the others.




==> include/Results2.tex <==
\section{Results}

\subsection{Datasets}

To test our method in an empirical experiment, we chose three datasets from three different stock market indices in different timeframes.
Descriptions of the datasets that we used can be observed in Table \ref{tab:datasets}.
The S\&P 500 data is available in daily resolution
The Nikkei 225 and S\&P 100 datasets were obtained from Indextrack datasets \cite{BEASLEY2003621}. The prices in this dataset are indexed from 0 to 291, which are the weekly prices between March 1992 to September 1997, and the train and test ranges are expressed as an index value in Table \ref{tab:datasets}.

\begin{table}[]
    \centering
   \caption{Datasets Information}
    \begin{tabularx}{0.45\textwidth}{|*{4}{c}}
    \hline
    
    \multicolumn{1}{|p{1.86cm}|}{Index} & \multicolumn{1}{p{1.86cm}|}{Asset Count} & \multicolumn{1}{p{1.86cm}|}{Train Range} & \multicolumn{1}{p{1.86cm}|}{Test Range} \\ \hline
    
    \multicolumn{1}{|p{1.86cm}|}{S\&P 500} & \multicolumn{1}{p{1.86cm}|}{465} & \multicolumn{1}{p{1.86cm}|}{2019-04-01 to 2019-08-01} & \multicolumn{1}{p{1.86cm}|}{2019-08-02 to 2019-09-01} \\ \hline
    
    \multicolumn{1}{|p{1.86cm}|}{Nikkei 225} & \multicolumn{1}{p{1.86cm}|}{225} & \multicolumn{1}{p{1.86cm}|}{0 to 200} & \multicolumn{1}{p{1.86cm}|}{201 to 290} \\ \hline
    
    \multicolumn{1}{|p{1.86cm}|}{S\&P 100} & \multicolumn{1}{p{1.86cm}|}{98} & \multicolumn{1}{p{1.86cm}|}{0 to 200} & \multicolumn{1}{p{1.86cm}|}{201 to 290} \\ \hline
    
    \end{tabularx}
    \label{tab:datasets}
\end{table}

\subsection{Metrics}

We used two approaches to evaluate the performance of the algorithms used in our paper. We measured the future performances of their output portfolios using several financial metrics and assessed their stability both in time and against noise via computational methods.

The financial ratios which we used to evaluate the future performance of portfolios were as following:

\begin{itemize}

\item Correlation: Since our method's primary focus was to minimize the correlation between different assets' price values, we must evaluate how minimization of correlation in train data relates to the correlation of portfolios in the test data. All of the other measures are a byproduct of this value.

\item Return: The return of the portfolios was evaluated in the test range.

\item Risk: The risk of the portfolios is defined as the standard deviation of the asset returns in a given time range.

\item Sharpe Ratio:
\begin{equation}
    Sharpe\ Ratio = \frac{R_{p} - r_{f}}{\sigma_{p}}
\end{equation}

Where $R_{p}$ is the return of the portfolio, $r_{f}$ is the risk-free rate of return, and $\sigma{p}$ is the standard deviation of the portfolio.

\item
Information Ratio:
\begin{equation}
 Information\ Ratio = \frac{R_{p} - R_{b}}{\sigma_{R_{p} - r_{b}}}     
\end{equation}

Where $R_{p}$ is return of the portfolio, $R_{b}$ is return of the benchmark, and $\sigma_{R_{p} - r_{b}}$ is the standard deviation of the excess return.

\item
M2 Measure (Modigliani):
\begin{equation}
 M2\ Measure = SR * \sigma_{b} + r_{f}   
\end{equation}
Where $SR$ is the Sharpe Ratio, $r_{f}$ is the risk-free rate of return, and $\sigma_{b}$ is the standard deviation of the benchmark.

\end{itemize}

To evaluate the stability of the algorithms, we took another approach.

\newtheorem{dfn}{Definition}
\begin{dfn}
Suppose that the training phase of an algorithm has resulted in $k_1$ different portfolios, where each is a set of assets. If the model is trained again under different circumstances, the result of the train would be $k_2$ portfolios. A stability matrix ($SM$) is defined as a $k_1 \times k_2$ matrix where $SM_{ij}$ is the similarity value between portfolio $i$ of the first train phase and portfolio $j$ of the second train phase.
\end{dfn}

The similarity metric we used in this paper was Jaccard Similarity measures, which is defined as below between set $A$ and set $B$:

\begin{equation}
    JaccardSim(A, B) = \frac{|A \cap B|}{|A \cup B|}
\end{equation}

Where $|S|$ is the size of set $S$. We use a matrix instead of a list because we cannot determine an injective function between two phases of training, and therefore no direct mapping exists between two sets of portfolios. After forming the stability matrix, we can extract different measures from it. First of all, we calculate the maximum similarity value for each portfolio to find a mapping between phases. One problem in this process is that the count of portfolios can vary between phases. For example, since the Louvain clustering algorithm does not provide input for several clusters, the output cluster count might differ in different training sets. Furthermore, some of the weighting algorithms might not reach a conversion point for a specific portfolio, and therefore the subset would not be present in the training process results. As a result of this problem, the column-wise maximum of the matrix is not necessarily equal to the row-wise maximum. We combine the row-wise and the column-wise maximums before any further inspections to create a symmetric measure from the similarity matrix.

After taking the maximums, we use the average of maximums to compute the stability of the algorithm. As mentioned before, we also use two different stability tests:

\begin{itemize}
    \item Noise Stability: The stability of the method if a minuscule amount of Gaussian noise is applied to the correlation matrix of the assets.
    \item Time Stability: The method's stability if the time range of the training dataset is shifted for a small amount.
\end{itemize}

Note that these stability functions cannot be applied to Random and Simulated Annealing selection methods since they are statistical approaches for the optimization problem and unstable. No two consecutive runs with similar conditions would result in the same portfolio using these methods.

\subsection{Experiments}

\paragraph{Future Performance} To measure the performance of RPS for each of the datasets that we had, we constructed several portfolios using different methods and compared their performances via the metrics that we described above. Firstly, we built a set of portfolios with a two-phased approach that used RPS for their asset selection in their first phase, and then used one of the portfolio optimization methods CLA \cite{niedermayer2010CLA}, MVO \cite{erlich2010MVO}, or HRP \cite{pfitzinger2019HRP}. Then we created a set of other portfolios using our benchmark methods. Three out of four of these methods, Mantegna (MTN), Random (RND), and Graph Splex (SPX), can be used in a two-phased fashion like ours. After computing the subsets, we used the same portfolio optimization methods mentioned above. The Simulated Annealing (SA) method is a one-phased method, and the result of its training contains the weights and portfolios. Furthermore, RPS and MTN methods result in multiple portfolios. We ran RND and SA multiple times to compare all of the benchmarks, but the SPX approach outputs a consistent result for a given market. Lastly, we could not run the SPX method on Nikkei 225 and S\&P 500 datasets since it did not converge on our systems in a bounded time.

The top 10 portfolios in the training range of each method were then picked, and their performances were evaluated in the test range. Portfolios were sorted using Sharpe value to maximize the return while minimizing the risk. The risk-return graph depicting the discussed portfolios can be observed in Figure \ref{fig:our_selection}.

\begin{figure}[!ht]
    \label{fig:our_selection}
    \centering
    \includegraphics[width=0.46\textwidth]{main/images/risk_return_idx4.png}
    \includegraphics[width=0.46\textwidth]{main/images/risk_return_idx5.png}
    \includegraphics[width=0.46\textwidth]{main/images/risk_return_sp500.png}
    \caption{The efficient-frontier plot for the top 10 portfolios of the training set for RPS+optimization versus benchmark algorithms.}
\end{figure}

Moreover, the best value of future metrics for each of the methods are available in Tables \ref{tab:sp500fp}, \ref{tab:nikkeifp}, and \ref{tab:sp100fp}.

\begin{table*}[!t]
  \centering
  \caption{Future Performance Measures for S\&P 500 Dataset}
  \begin{tabular}{ccccccc}
    \hline
    Method & Correlation & Return & Risk & Sharpe Ratio & Information Ratio & M2 \\
    \hline
    Vanilla CLA & 0.162075 & 0.027747 & 0.114838 & 0.164118 & 0.242098 & 0.027636  \\
    RPS+CLA & 0.138791 & \textbf{1.110586} & 0.369897 & 3.435445 & \textbf{4.721627} & 0.817560 \\
    MTN+CLA & 0.196280 & 1.094718 & 0.369051 & \textbf{4.948828} & 4.654215 & \textbf{1.173791} \\
    RND+CLA & 0.171342 & 0.267575 & 0.535209 & 1.031657 & 1.140248 & 0.251739 \\
    \hline
    Vanilla HRP & 0.162075 & 0.011727 & \textbf{0.095295} & 0.216459 & 0.103681 & 0.015811  \\
    RPS+HRP & \textbf{0.008178} & 0.535214 & 0.269456 & 2.153089 & 2.277263 & 0.515710 \\
    MTN+HRP & 0.196280 & 0.541221 & 0.270475 & 3.698830 & 2.302783 & 0.879557  \\
    RND+HRP & 0.191148 & 0.166312 & 0.291356 & 0.773329 & 0.710050 & 0.190932 \\
    \hline
    Vanilla MVO & 0.162075 & 0.027747 & 0.114838 & 0.164118 & 0.242098 & 0.027636  \\
    RPS+MVO & 0.138791 & 0.932556 & 0.285581 & 4.163090 & 3.965298 & 0.988838 \\
    MTN+MVO & 0.235134 & 0.557674 & 0.215301 & 3.736161 & 2.372682 & 0.888345 \\
    RND+MVO & 0.174462 & 0.165436 & 0.262077 & 0.597288 & 0.706327 & 0.149494 \\
    \hline
    SA & 0.167465 & 0.273648 & 0.210593 & 1.117717 & 1.166047 & 0.271996  \\ \hline
  \end{tabular}
  \label{tab:sp500fp}
\end{table*}

\begin{table*}[!t]
  \centering
  \caption{Future Performance Measures for Nikkei 225 Dataset}
  \begin{tabular}{ccccccc}
    \hline
    Method & Correlation & Return & Risk & Sharpe Ratio & Information Ratio & M2 \\
    \hline
    Vanilla CLA & 0.450845 & 0.143052 & 0.436134 & 0.261482 & 0.278425 & 0.142717  \\
    RPS+CLA & \textbf{0.094671} & \textbf{1.991665} & 0.387936 & 3.818792 & \textbf{4.599676} & 1.665158 \\
    MTN+CLA & 0.210820 & 0.395800 & 0.403417 & 0.790543 & 0.920129 & 0.351768 \\
    RND+CLA & 0.189425 & 0.962127 & 0.398781 & 2.390352 & 2.225895 & 1.045625 \\
    \hline
    Vanilla HRP & 0.450845 & 0.042383 & 0.422741 & 0.069599 & 0.081713 & 0.044518  \\
    RPS+HRP & 0.176072 & 0.165529 & 0.403649 & 0.385897 & 0.389200 & 0.176268 \\
    MTN+HRP & 0.210820 & 0.946481 & 0.354701 & 2.427145 & 2.189820 & 1.061583 \\
    RND+HRP & 0.265348 & -0.411154 & 0.405019 & -1.037120 & -0.940445 & -0.440912 \\
    \hline
    Vanilla MVO & 0.450845 & 0.143052 & 0.436134 & 0.261482 & 0.278425 & 0.142717  \\
    RPS+MVO & \textbf{0.094671} & 1.978367 & 0.400116 & \textbf{3.826142} & 4.569014 & \textbf{1.668345} \\
    MTN+MVO & 0.210820 & 0.594692 & \textbf{0.352680} & 1.520505 & 1.378710 & 0.668362 \\
    RND+MVO & 0.105741 & -0.315837 & 0.374047 & -0.868171 & -0.720674 & -0.367636 \\
    \hline
    SA & 0.558230 & -0.937416 & 0.420207 & -2.070724 & -2.153834 & -0.889199 \\
    \hline
  \end{tabular}
  \label{tab:nikkeifp}
\end{table*}

\begin{table*}[!t]
  \centering
  \caption{Future Performance Measures for S\&P 100 Dataset}
  \begin{tabular}{ccccccc}
    \hline
    Method & Correlation & Return & Risk & Sharpe Ratio & Information Ratio & M2 \\
    \hline
    Vanilla CLA & 0.418337 & 1.269428 & 0.198022 & 4.348930 & 4.385291 & 1.262862 \\
    RPS+CLA & 0.177503 & 2.783124 & 0.481028 & 4.457300 & 9.635014 & 1.294110 \\
    MTN+CLA & 0.155783 & 2.630134 & 0.402634 & 4.461950 & 9.104422 & 1.295450 \\
    SPX+CLA & 0.870104 & 2.461136 & 0.571726 & 4.289180 & 8.518312 & 1.245634 \\
    RND+CLA & 0.208234 & \textbf{3.696725} & 0.320223 & \textbf{5.226347} & \textbf{12.803521} & \textbf{1.515855} \\
    \hline
    Vanilla HRP & 0.418337 & 1.278512 & 0.195795 & 4.449693 & 4.416796 & 1.291916 \\
    RPS+HRP & 0.255930 & 1.473516 & 0.257972 & 3.724968 & 5.093098 & 1.082950 \\
    MTN+HRP & 0.155783 & 2.100452 & 0.298370 & 4.351074 & 7.267409 & 1.263480 \\
    SPX+HRP & 0.870104 & 2.585765 & 0.627108 & 4.109122 & 8.950544 & 1.193717 \\
    RND+HRP & 0.206733 & 1.548159 & \textbf{0.252117} & 4.243590 & 5.351972 & 1.232489 \\
    \hline
    Vanilla MVO & 0.418337 & 1.269428 & 0.198022 & 4.348930 & 4.385291 & 1.262862 \\
    RPS+MVO & 0.177503 & 2.790539 & 0.481578 & 4.476027 & 9.660732 & 1.299509 \\
    MTN+MVO & 0.339761 & 1.914374 & 0.303960 & 4.823667 & 6.622061 & 1.399747 \\
    SPX+MVO & 0.870104 & 2.461136 & 0.571726 & 4.289180 & 8.518312 & 1.245634 \\
    RND+MVO & \textbf{0.043606} & 1.634323 & 0.306306 & 4.889193 & 5.650800 & 1.418641 \\
    \hline
    SA & 0.217874 & 1.759462 & 0.326334 & 4.851917 & 6.084802 & 1.407893 \\
    \hline
  \end{tabular}
  \label{tab:sp100fp}
\end{table*}

It can be seen in these tables that in S\&P 500 and Nikkei 225, RPS has reached the best possible return among other methods and also the best correlation value. It can be seen that selection in all of the instances caused the correlation value to decrease from the original correlation of the assets. However, the results of performances are pretty different in S\&P 100 database. It is consistent with the notion that a random selection phase can lead to relatively high-performance portfolios since it can reach any point in the space of portfolios. The relative lousy performance of all other algorithms can be explained by looking at the correlation of all the assets in the dataset. The overall average correlation between assets of S\&P 100 is equal to 0.418337. Since the market assets are highly correlated, it becomes harder for the selection algorithms to find a highly uncorrelated subset, and therefore, most of the portfolios would move in the direction of the general trend. Both good performance of selection algorithms and bad performance of random selection in Nikkei 255 and bad performance of selection algorithms and good performance of random selection in S\&P 100 can be explained using this argument. Moreover, we can inspect the return of all portfolios in the markets in Figure \ref{fig:return_dist}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{main/images/returns_dist_idx4.png}
    \includegraphics[width=0.47\textwidth]{main/images/returns_dist_idx5.png}
    \includegraphics[width=0.47\textwidth]{main/images/returns_dist_sp500.png}
    \caption{Return distribution}
    \label{fig:return_dist}
\end{figure}

It can be seen in Figure \ref{fig:return_dist} that RPS achieves a higher average return. In S\&P 100, few of the RND portfolios were able to reach a high return value, and also SPX achieves a higher average return, but as can be seen in the figure, RPS can obtain higher average performance.

\paragraph{Stability} The time and noise stability metrics are shown in table \ref{tab:ns} and \ref{tab:ts}. Gaussian noise with $\mu=0$ and $\sigma=0.01$ was applied to the market correlation matrix for noise stability. For time stability, the train time ranges were shifted to 20 data points for each dataset.

\begin{table}[!hbtp]
  \centering
  \caption{Noise Stability}
  \begin{tabular}{cccc}
    \hline
    Method & S\&P 100 & Nikkei 225 & S\&P 500 \\ \hline
    Mantegna & \textbf{0.528711} & \textbf{0.479277} & \textbf{0.427159} \\
    RPS & 0.460720 & 0.373794 & 0.085135 \\
    Splex & 0.000000 & - & - \\
    \hline
  \end{tabular}
  \label{tab:ns}
\end{table}

\begin{table}[!hbtp]
  \centering
  \caption{Time Stability}
  \begin{tabular}{cccc}
    \hline
    Method & S\&P 100 & Nikkei 225 & S\&P 500 \\ \hline
    Mantegna & 0.336598 & \textbf{0.360965} & \textbf{0.228190} \\
    RPS & \textbf{0.557390} & 0.231124 & 0.119387 \\
    Splex & 0.400000 & - & - \\
    \hline
  \end{tabular}
  \label{tab:ts}
\end{table}

In noise stability metrics, MTN was able to outperform RPS and SPX methods. However, the margin of superiority was not significant in the S\&P 100 dataset, resulting from the smaller size of the database and the lower number of options available in the selection phase. As the size of the dataset grows, stability drops for all of the methods.

\paragraph{RPS Clustering Method} Another issue to analyze is whether the clustering method (k-means or fuzzy c-means) affects outcoming portfolios or not. Figure \ref{fig:rps_cluster} depicts the risk-return relation for all different setups of RPS ran in the test range.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{main/images/rps_cluster_method.png}
    \caption{Risk-Return distribution of RPS on S\&P 500 dataset, separated by clustering method.}
    \label{fig:rps_cluster}
\end{figure}

As seen in this figure, there are no significant differences between the portfolios using these two clustering methods.

==> include/abstract.tex <==
% As a general rule, do not put math, special symbols or citations
% in the abstract
\begin{abstract}
Portfolio optimization is one of the essential fields of focus in finance. There has been an increasing demand for novel computational methods in this area to compute portfolios with better returns and lower risks in recent years. We present a novel computational method called Representation Portfolio Selection (RPS) by redefining the distance matrix of financial assets using Representation Learning and Clustering algorithms for portfolio selection to increase diversification. RPS proposes a heuristic for getting closer to the optimal subset of assets. Using empirical results in this paper, we demonstrate that widely used portfolio optimization algorithms, such as MVO, CLA, and HRP, can benefit from our asset subset selection.
\end{abstract}

==> main/include/Conclusion.tex <==
\section{Conclusion}

This paper aimed to provide a new portfolio selection method that could outperform other algorithms used in the portfolio asset selection phase. To fulfill our goals, we provided a novel portfolio selection method based on representation learning and graph embedding called RPS. As seen in the results, various portfolio weight optimization methods can benefit from using RPS, since in every instance, using RPS selection improved the overall performance of the method versus the vanilla usage of that method. We have also seen that the portfolios constructed by RPS have a generally higher return than their rivals. Future directions can add dynamics to the problem and consider changing portfolios in time by periodic training RPS. Other weight optimization methods can also be tested on the selection to improve the portolios' performance further.

==> main/include/Evaluation.tex <==
\section{Evaluation Benchmark}

\paragraph{Minimum Spanning Tree (MST) and Hierarchical Clustering} The approach described in \cite{mantegna99paper} uses Kruskal's algorithm to build an MST over the complete graph of the market. The edges' weights are determined by the relation below.

\begin{equation}
d_{ij} = \sqrt{2(1 - \rho_{ij})}
\end{equation} 

where $\rho_{ij}$ is the correlation between asset $i$ and asset $j$. This approach relaxes the market graph and makes it easier for further operations. The paper itself does not specify a way to reach subsets of assets. We use Louvain Clustering Algorithm \cite{Blondel_2008} to extract smaller subsets of the market for evaluation. The clusters can be given to a weighting method, similar to RPS.

\paragraph{Graph Splex} The Graph Splex \cite{splex} tries to reach a diversified portfolio by creating a clique-like substructure of the market assets. We implemented this method using the pseudo-code described in the body of \cite{splex}. This subdivision can be weighted using the weight methods.

\paragraph{Simulated Annealing} Overall, various hill-climbing algorithms can be used as the solution for portfolio optimization cardinality problems, such as Simulated Annealing and Genetic Algorithms. The method starts with a random set of states for a subset of assets and changes the weights until a stable state is reached \cite{crama-schyns03, maringer05}.

\paragraph{Random Subsets} Since our goal is to constraint the cardinality of assets, we can use random divisions of the market as a baseline method. In this approach, Since random subdivision has access to every market subset, there is a probability that it can reach some of the best baskets. After selecting this subdivision, we can run the optimization methods on the portfolios.

==> main/include/FutureWorks.tex <==
\section{Future works}
% \begin{itemize}
%     \item Perioding?
%     \item Dynamic of portfolio
%     \item Preferences?
%     \item Other datasets (like tweets)
%     \item Graph representation with supervision or other data
% \end{itemize}
Our proposed model finds portfolio weights based on a fixed training period and suggest buying stock shares for the next period. One future direction would be to alter the model to offer buy/sell signals in real-time to achieve a more actionable model. This way, we could also consider other trading constraints and complexities like trade limits and trading costs. Additionally, our model just uses price time series to find relationship between different shares. We could also leverage news articles or related tweets sentiments as another source of information. Finally, the graph representation learning module used in this work is an unsupervised learning method that finds underlying relations between shares. Using supervisionfrom the next periods, we could enable the model to learn price dynamics and consider these dynamics in finding share similarities that are optimized for future periods.

==> main/include/Introduction-2.tex <==
For decades, Portfolio construction and optimization have had investors' attention. Financial institutions have long been pursuing methods to increase their returns further while also controlling their risks.

In this paper, we try to address this matter by proposing a two-phased portfolio construction method. This method first selects a subset of assets and then weights the obtained assets. While many portfolio optimization methods do not select the assets explicitly before weighing them, we focus on portfolio selection in this paper. We will indicate that we will reach better portfolios with higher returns and less risk by separating the portfolio asset selection phase from the portfolio weighting phase. Furthermore, we state that doing so would help us to overcome multiple issues. Firstly, it eliminates the covariance estimation inaccuracy which exists in previous portfolio optimization methods. Secondly, it resolves portfolio optimization algorithms such as MVO, which would have convergence problems if given an extensive benchmark of assets by pre-selecting a heuristically optimal subset of assets.

On its own, Portfolio construction is a classic research field in the finance area. However, with the growing influence of computational and machine learning methods, it can perhaps be seen from another perspective as an intermediary field. With that in mind, creative computational methods for this classic problem will start to rise. We are presenting in this paper is a novel method for stock selection using representation learning methods.
For portfolio selection and, more generally, portfolio construction, asset similarity plays a substantial role. Experts measure the similarity between assets in different ways, namely correlation, covariance, and granger causality (See, e.g.,   \cite{akhtaruzzaman2020influence,berger2020short,apergis2021cyclicality}). Whatever the measurement for the similarity may be, the ultimate goal is to reach diversification in portfolios by selecting uncorrelated assets for them.


In this paper, we redefine the similarity measurement of pairwise assets by defining a new distance for assets based on their correlation matrix by using Node2Vec. Moreover, with these sets of distances in our new embedding space, an uncorrelated set of assets can be selected using clustering methods. This procedure gives us a subset of assets that we can assign weights to the selected assets using a portfolio optimization algorithm. 

This paper will provide portfolio optimization algorithms a subset of assets using our portfolio selection method, which we will call RPS (Representation Portfolio Selection), and we will show that using our subset asset selection method, a portfolio optimization method's performance can be enhanced.  We applied RPS to widely used portfolio optimization algorithms such as CLA, HERC, HRP, and MVO, and for each of them, we observed that RPS improved their performance.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=\textwidth]{main/images/method diagram.png}
    \caption{Stages of RPS algorithm.}
    \label{fig:methoddiagram}
\end{figure*}

\input{main/include/RelatedWorks-2}

==> main/include/Introduction-3.tex <==
For decades, Portfolio construction and optimization have had investors’ attention. Financial institutions have long been pursuing methods to increase their returns further while also controlling their risks. The main goal in Portfolio Construction is to select a set of assets from a variety of  asset classes, and allocate investment weights to them, with the objective to maximise the overall investment return based on the given investment strategy and risk profile. The rather holistic approach of Portfolio Construction, aims to create a consistent flow of return in the long term, and to protect the investor from the market downturns, thus making Portfolio Construction methodologies valuable to numerous financial institutions and investors.

Over the course of time, lots of different techniques and approaches formed to address the issue of portfolio optimization. One of the first and most famous theories was Markowitz’s Portfolio Theory [cite, 1952]. In his study, he utilized the covariance matrix of the financial assets to define the problem as a quadratic programming problem. The success of Markowitz’s theory embarked on the creation of many other methods in this field, and in fact most of portfolio construction and optimization methods have used the core idea of Markowitz’s theory, which is tha the lower the correlation of a portfolio's assets, the lower the risk of that portfolio. To point out a few successful portfolio construction methods based on Markowitz modern portfolio theory, we can name CLA [2013, cite] and MVO [cite]. There are also some other well-known approaches that are based on computational algorithms such as clustering, including HRP [cite], HERC [cite], and NCO [cite].

Moreover, a body of literature investigates the portfolio selection method, which is to select a subset of assets that are a good choice set for portfolio construction. This was done both by using network methods like finding spanning trees on correlation-based graphs \cite{mantegna1999hierarchical} \cite{tumminello2010correlation} and other clustering methods like k-means and hierarchical clustering \cite{lemieux2014clustering} \cite{raffinot2017hierarchical} \cite{leon2017clustering}.

While portfolio construction is a classic research field in the finance area, with the growing influence of computational and machine learning methods, it can be seen from another perspective as an intermediary field. With that in mind, creative computational methods for this classic problem will start to rise. Some methods first predict each asset changes in the future and use the results for portfolio construction \cite{ta2018prediction}, \cite{chen2021mean}  \cite{ma2021portfolio}. Other methods have been also used to directly construct the portfolios by training on previous data, such as Reinforcement Learning \cite{yu2019model}, and Deep Learning \cite{2005.13665}. A core characteristic of the asset markets, in general, is the complexity of them. Having a robust way to deal with this complexity will be useful to solve the portfolio optimization problem. One of the machine learning methods that can be used to do so is Representation learning, which is a learning method that embeds the entities in the problem in a low-dimensional feature space. For instance, \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method is able to identify groups of stocks that had similar price behavior as well as similar news. On the other hand, \cite{hu2018deep} uses candlestick images and image neural network architectures to reach a proper representation for each stock.

In this paper, we try to address this matter by using a representation method on asset similarity graphs, which we construct using the correlation matrix of assets. We leverage these representations in a two-phased portfolio optimization setting. We select a subset of assets first and then weight the obtained assets. While many portfolio optimization methods do not select the assets explicitly before weighing them, we focus on portfolio selection in this paper. We will indicate that we will reach better portfolios with higher returns and less risk by separating the portfolio asset selection phase from the portfolio weighting phase. Furthermore, we state that doing so would help us to overcome multiple issues. Firstly, it eliminates the covariance estimation inaccuracy which exists in previous portfolio optimization methods. Secondly, it resolves portfolio optimization algorithms such as MVO, which would have convergence problems if given an extensive benchmark of assets by pre-selecting a heuristically optimal subset of assets.

% There are variety of machine learning methods used for constructing portfolios. Some methods leverage optimization methods to overcome computational and estimation problems of portfolio optimization methods. \cite{still2010regularizing} uses a regularization method to construct weights that are stable and robust to fluctuations. \cite{perrin2020machine} investigates optimization methods to find a method that could be practically used for real-world problems with lots of assets. Some other studies, use prediction models to first predict each assets future dynamics and then use the predictions to find optimal assets. \cite{ta2018prediction}, \cite{chen2021mean}, \cite{ma2021portfolio} investigate a range of machine learning methods from simpler methods (Linear Regression \& Support Vector Regression) to more complex methods (XGBoost \& LSTMs). RL methods have also been studied, in which an agent learns how to construct appropriate portfolios by behaving in the environment \cite{yu2019model}.

% Moreover, representation learning methods have also been studied for portoflio optimization recently. For instance, \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method is able to identify groups of stocks that had similar price behavior as well as similar news. On the other hand, \cite{hu2018deep} uses candlestick images and image neural network architectures to reach a proper representation for each stock.


%We design the method is a way that the distance measure in the embedding space would represent how much the two assets are correlated.

% 

% In this paper, we try to address this matter by using a representation method on asset similarity graph. We leverage these representations in a two-phased portfolio optimization setting. We select a subset of assets first and then weight the obtained assets. While many portfolio optimization methods do not select the assets explicitly before weighing them, we focus on portfolio selection in this paper. We will indicate that we will reach better portfolios with higher returns and less risk by separating the portfolio asset selection phase from the portfolio weighting phase. Furthermore, we state that doing so would help us to overcome multiple issues. Firstly, it eliminates the covariance estimation inaccuracy which exists in previous portfolio optimization methods. Secondly, it resolves portfolio optimization algorithms such as MVO, which would have convergence problems if given an extensive benchmark of assets by pre-selecting a heuristically optimal subset of assets.

% For portfolio selection and, more generally, portfolio construction, asset similarity plays a substantial role. Experts measure the similarity between assets in different ways, namely correlation, covariance, and granger causality (See, e.g.,   \cite{akhtaruzzaman2020influence,berger2020short,apergis2021cyclicality}). Whatever the measurement for the similarity may be, the ultimate goal is to reach diversification in portfolios by selecting uncorrelated assets for them.

% In this paper, we redefine the similarity measurement of pairwise assets by defining a new distance for assets based on their correlation matrix by using Node2Vec. Moreover, with these sets of distances in our new embedding space, an uncorrelated set of assets can be selected using clustering methods. This procedure gives us a subset of assets that we can assign weights to the selected assets using a portfolio optimization algorithm. 

% This paper will provide portfolio optimization algorithms a subset of assets using our portfolio selection method, which we will call RPS (Representation Portfolio Selection), and we will show that using our subset asset selection method, a portfolio optimization method's performance can be enhanced.  We applied RPS to widely used portfolio optimization algorithms such as CLA, HERC, HRP, and MVO, and for each of them, we observed that RPS improved their performance.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=\textwidth]{main/images/method diagram.png}
    \caption{Stages of RPS algorithm.}
    \label{fig:methoddiagram}
\end{figure*}

\input{main/include/RelatedWorks-3}

==> main/include/Introduction-4.tex <==
\section{Introduction}
Deciding how and where to invest money is one of the main challenges anyone with some savings faces. The complexity of finding an answer to this challenge has increased as the options for investment have grown in time, from gold and land to a myriad of financial assets like stocks, currencies, and cryptocurrencies. Moreover, investing money will be more important when the amount of money is considerable, such as for financial institutes, where any wrong decision or any fluctuation in the price of the invested asset can lead to considerable losses. In this situation, each individual can decide how to invest their money based on different parameters like knowledge, beliefs, and future predictions.

Two crucial concepts help investors diversify their assets. First is constructing an initial portfolio, which is a collection of financial assets that one individual holds. The second is managing the portfolio afterward. While these two concepts are interlinked, the dynamics of assets and trading constraints in markets introduce more complexities than the former, making them two different problems to solve. This paper will focus on the first problem, portfolio construction, and leave analyzing the complexities of portfolio management to future studies. Studies on the portfolio optimization problem have a long history. One of the first and most famous theories that studied portfolio construction was Markowitz's Portfolio Theory \cite{markowitz52, markowitz59, markowitz87}, which became the cornerstone of modern portfolio theory. In his study, he utilized the covariance matrix of the financial assets to define the problem as a quadratic programming problem. The success of Markowitz's theory embarked on creating many other methods in this field with different ideas. However, most portfolio construction and optimization methods have used the core idea of Markowitz's theory: the lower the correlation of a portfolio's assets, the lower the risk. Although naturally, many papers started studying the shortcomings of Markowitz's methods and addressed solutions to those shortcomings \cite{eltongruber95, king93, konnoyamazaki91, milis97, mitra2003review, rockafellar2000optimization}.

One of the Markowitz issues that we mitigate in this paper is the cardinality constraint problem. Markowitz’s method outputs the fraction of money to invest on each asset, with the assets and price history as the input. There are thousands of various assets available for investment, which can lead to hardships since managing such portfolios can be complicated. Moreover, it can be shown that limiting assets to a maximum count is a form of the Knapsack problem, which is computationally NP-hard \cite{garey-johnson79}. Different methods use different types of heuristics to solve this issue. For example, Crama and Schyns \cite{crama-schyns03} and Maringer \cite{maringer05} used simulated annealing, while others use clustering methods like k-means and hierarchical clustering \cite{lemieux2014clustering, raffinot2017hierarchical, leon2017clustering}. A whole family of other solutions formed based on Mantegna’s Minimum Spanning Tree method \cite{mantegna99book, mantegna99paper}. Some other methods try to reformulate the problem and solve it mathematically, such as Cesarone et al. \cite{Cesarone2013ANM}.

With the growing influence of computational and machine learning methods on financial markets, portfolio construction can be seen as an intermediary field from another perspective. A variety of computational methods have started to rise. Some methods first predict each asset changes in the future and use the results for portfolio construction \cite{ta2018prediction, chen2021mean, ma2021portfolio}. Other methods have also been used to directly construct the portfolios by training on previous data, such as Reinforcement Learning \cite{yu2019model}, and Deep Learning \cite{zhang2020deep}. A core characteristic of the asset markets, in general, is their complexity. Having a robust way to deal with this complexity will be useful to solve the portfolio optimization problem. One of the machine learning-based methods that can be used to do so is Representation learning, which is a learning method that embeds the entities in the problem in a low-dimensional feature space. For instance, \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method can identify groups of stocks that had similar price behavior as well as similar news. On the other hand, \cite{hu2018deep} uses candlestick images and image neural network architectures to obtain a proper representation for each stock.

A new family of representation learning methods has formed in recent years, which embed the nodes of the graphs using their connections. This paper addresses the portfolio construction problem using the Node2Vec \cite{grover2016node2vec} method, a graph representation learning algorithm, on asset similarity graphs using the correlation matrix of assets. We leverage these representations in a two-phased portfolio optimization setting. First, we select a subset of assets and then weigh the obtained assets. While many portfolio optimization methods do not select the assets explicitly before weighing them, we focus on portfolio selection in this paper. We will indicate that better portfolios with higher returns and less risk can be achieved by separating the portfolio asset selection phase from the portfolio weighting phase. Furthermore, we state that doing so would help us to overcome multiple issues. Firstly, it eliminates the covariance estimation inaccuracy which exists in previous portfolio optimization methods. Secondly, it resolves portfolio optimization algorithms such as Mean-Variance Optimization (MVO) \cite{erlich2010MVO}, which would have convergence problems if given an extensive benchmark of assets by pre-selecting a heuristically optimal subset of assets.

 The paper is organized in the following structure.  Section II provides an in-depth description of the proposed method.  Section III discusses the other baseline methods that can be used for the portfolio selection problem.  At last, the results of the evaluation on multiple datasets are provided in section IV.


==> main/include/Introduction.tex <==
\section{Introduction}
% \begin{itemize}
%     \item What is the portfolio optimization problem?
%     \item What are the already available solutions?
%     \item Previous works problems.
%     \item What is our proposed solution?
%     \item Why is our method, good?
%     \item Structure of the paper.
% \end{itemize}
For decades, Portfolio construction and optimization has had the attention of investors, financial institutions have long been pursuing methods to further increase their returns, while also controlling their risks. 
Portfolio construction has two main key parts, the first part is asset selection, and the second part is weighting the assets held in the portfolio. Weighting a given benchmark of assets implicitly also includes Portfolio selection. In other words, many portfolio optimization methods do not select the assets explicitly before weighting them. In this paper, we separate these two parts and focus on the portfolio selection process, and indicate that pre-selection of benchmark and weighting the selected subset of assets afterward reaches better results.
On its own, Portfolio construction is a classic financial research area, but with the growing influence of computational methods and machine learning over other fields, it can perhaps be seen from another perspective, as an intermediary field, and with that in mind, creative computational methods for this classic problem will start to rise. That is what we are presenting in this paper, a novel method for stock selection using representation learning.
For portfolio selection and more generally, portfolio construction, asset similarity plays a substantial role. The similarity between assets can be and has been measured in different ways, namely correlation, Covariance, and Granger causality [reference papers]. Different approaches have been taken before, but whatever the measurement for the similarity may be, the ultimate goal is to reach diversification in our portfolio by selecting uncorrelated assets for the portfolio.
In this paper, we redefine the similarity measurement of pairwise assets by defining a new distance for each pair of assets based on their correlation matrix, by using Node2Vec. And with these sets of distances in our new embedding space, an uncorrelated set of assets can be selected by using clustering methods. This gives us a subset of assets that we can assign weights to the selected assets using a portfolio optimization algorithm. 
In this paper, we will provide portfolio optimization algorithms a subset of assets using our portfolio selection method, which we will call RPS (Representation Portfolio Selection), and we will show that using our subset asset selection method, a portfolio optimization method's performance can be enhanced.  We applied RPS to widely used portfolio optimization algorithms such as CLA, HERC, HRP, and MVO, and for each of them, we observed that RPS improved their performance.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.8\textwidth]{templates (1)/images/method diagram.png}
    \caption{Stages of RPS algorithm.}
    \label{fig:methoddiagram}
\end{figure*}

\input{templates (1)/include/RelatedWorks}

==> main/include/Method-2.tex <==
\section{Method}

This paper aims to present a novel utilization of representation learning as a diversification heuristic for a portfolio. The main idea is to choose uncorrelated assets for a portfolio to minimize the portfolio variance, which means less risk for the portfolio.
To elaborate, take $N$ assets in a portfolio which are pairwise uncorrelated, i.e., $\forall i \neq j, \rho_{i j}=0 .$ Then the variance for this portfolio would be 

$$
Var\left(P\right)=\sum_{i=1}^{N}\left(w_{i}\right)^{2} \sigma_{i}^{2}
$$


And to better show the idea, with the simplifying assumption of equal weights for the assets, i.e., $i, w_{i}=1 / N,$ we will have

$$
Var\left(P\right)=\frac{1}{N^{2}} \sum_{i=1}^{N} \sigma_{i}^{2} \leq \frac{\sigma_{M}^{2}}{N}
$$
where $$ \sigma_{M}=\max \left[\sigma_{i}: i=1, \ldots, N\right]$$

And as $N$ grows to infinity, $Var\left(P\right)$ will lean towards $0$. This shows us that the more pairwise uncorrelated assets we have in our portfolio, the smaller the portfolio's risk will be. Even though we do not have completely uncorrelated assets in real life, we can still build upon the shown idea and choose rather uncorrelated assets to reach a well-diversified low-risk portfolio. In this paper, we would want to build an augmented graph with some properties out of these assets based on their similarity or, to be more exact, their pairwise correlation, and then by applying a representation learning method on the graph, reach a new distance representation for the assets, which we can then choose the uncorrelated assets from to fulfill the idea shown above. 


To use machine learning and deep learning methods on graph-structured data, we must first embed the graph or its nodes in a vector space. There are different types of methods being used for this purpose. Some of them use discrete metrics to define the similarity between nodes like the number of common neighbors \cite{ahmed2013distributed, cao2015grarep}. Others use random walks, and the probability of observing one node while starting from another node as the similarity of the two nodes \cite{perozzi2014deepwalk, grover2016node2vec}. These two methods are unsupervised and do not require any labels on data. However, if we have some labeled data, we can employ other methods that utilize the labels to find better representations. These methods have been improved by using other properties of graphs \cite{kipf2016semi, hamilton2017inductive}. Since our data is unlabeled and our initial metric (correlation) was not discrete, we chose to use Node2Vec and apply it on the correlation graph of the stocks that we constructed to reach a new similarity metric so that ultimately we can select a set of stocks which gives us a diversified portfolio.

To build the described graph, we first need to set weights for the edges. We chose Pearson correlation as the basis of the pairwise similarity measure for the assets, and then we had to adjust the measurement for better results. As for the adjustment and why it is needed since we will be applying Node2Vec to the graph and as it is a random walk based algorithm on the weights of our graph, at a given node, it will iterate through the edge $j $ with a probability of $ \frac{w_{j}}{\sum_{i=1}^{n} w_{i}}$. So we have to augment the basic Pearson Correlation such that the more correlated the two assets are, the less the weight of their intermediate edge will be and vice versa. After applying Node2Vec, starting a random walk on a node, results in more visits to uncorrelated assets. Furthermore, to ensure that we will not be visiting high correlated assets for a starting node in a Node2Vec with a walk length of greater than 1, we should also consider these properties in our transformation function:

\begin{itemize}
    \item 
    As the corresponding correlation of an edge approaches 0, the edge's weight should approach infinity.
    \item
    As the corresponding correlation of an edge approaches 1, the edge's weight should approach 0.
\end{itemize}

We used hyperbolic cotangent for our weight adjustment as it supported such properties. Then, The new redefinition of pairwise similarity between assets which was also used as the weight of the edges in our graph is calculated this way:

\begin{equation}
w_{ij} = \mid \coth(Correlation(i,j)) \mid -\coth(1)
\end{equation}

\begin{figure}[]
    \centering
    \includegraphics[width=0.5\textwidth]{main/images/method_diagram.png}
    \caption{Stages of RPS algorithm.}
    \label{fig:methoddiagram}
\end{figure}

As our graph is built, the next step is to run Node2Vec on our graph. For each node, multiple random walks are executed based on the weights of its edges. That is, in each step, the algorithm visits the neighbor $j$ of a starting node with a probability of $ \frac{w_{j}}{\sum_{i=1}^{n} w_{i}}$, where $w_j$ is the weight of the edge between the starting node and neighbor $j$, and the algorithm iterates over the graph in this manner $l$ times for each execution, where $l$ is the walk-length of the algorithm. In the end, a new pair-wise distance representation is created based on the nodes visited during the execution of the algorithm for each starting node. Since we built the graph so that the edges with corresponding uncorrelated nodes to have greater weight than correlated ones, we will visit uncorrelated nodes for each node after this algorithm.

After embedding the nodes of the graph, we are free to use different clustering algorithms to reach our final portfolios. We used two different clustering methods. The first one was the k-means clustering algorithm, and the second one was the fuzzy c-means algorithm, which allows each node to be present in more than one subset. Our initial belief was that this relaxation might allow the procedure to achieve better performance. Since our representation of the graph is produced so that the uncorrelated assets are closer to each other, we will reach clusters of relatively uncorrelated assets, which can be interpreted as selected assets for our diversified portfolio.

The last step in the method is to input the resulted portfolios into a portfolio optimization method to calculate the fraction of wealth to invest in each of them. In this paper, we made use of three different optimization methods: MVO \cite{erlich2010MVO}, Hierarchical Risk Parity (HRP) \cite{pfitzinger2019HRP}, and Critical Line Algorithm (CLA) \cite{niedermayer2010CLA}.

==> main/include/Method.tex <==
\section{Method}
Our goal in this paper is to present a novel utilization of representation learning as a diversification heuristic for a portfolio. The main idea is to choose uncorrelated assets for a portfolio so that we can minimize the portfolio variance which means less risk for the portfolio.
To elaborate, take $N$ assets in a portfolio which are pairwise uncorrelated, i.e., $\forall i \neq j, \rho_{i j}=0 .$ Then the variance for this portfolio would be 

$$\operatorname{Var}\left(P\right)=\sum_{i=1}^{N}\left(w_{i}\right)^{2} \sigma_{i}^{2}$$


And to better show the idea, with the simplifying assumption of equal weights for the assets, i.e., $i, w_{i}=1 / N,$ we will have

$$
\operatorname{Var}\left(P\right)=\frac{1}{N^{2}} \sum_{i=1}^{N} \sigma_{i}^{2} \leq \frac{\sigma_{M}^{2}}{N}
$$
where $$ \sigma_{M}=\max \left[\sigma_{i}: i=1, \ldots, N\right]$$

And as $N$ grows to infinity,  $\operatorname{Var}\left(P\right)$  will lean towards $0 .$ This shows us, that the more pairwise uncorrelated assets we have in our portfolio, the smaller the risk of the portfolio will be. Even though we do not have completely uncorrelated assets in real life, we can still build upon the shown idea and choose rather uncorrelated assets to reach a well diversified low risk portfolio. In this paper, we would want to build an augmented graph with some properties out of these assets based on their similarity or to be more exact, their pairwise correlation, and then by applying node2vec on the graph, reach a new distance representation for the assets, which we can then choose the uncorrelated assets from to fulfil the idea shown above. 


To build the described graph, we first need to set weights for the edges. For this task we first need a pairwise similarity measure for the assets and then we have to adjust the measurement for better results. We chose Pearson correlation for as the basis of the similarity measurement, as our data was internal and correlation is [\todo{give reasons for correlation}]. As for the adjustment and why it is needed, since we will be applying node2vec to the graph and as it is a random walk based algorithm on the weights of our graph, at a given node, it will iterate through the edge $j $ with a probability of $ \frac{w_{j}}{\sum_{i=1}^{n} w_{i}}$. So we have to augment the basic Pearson Correlation such that the more correlated the two assets are, the less the weight of their intermediate edge should be and vice versa. This way after applying node2vec, starting a random walk on a node, results in more visits to uncorrelated assets. Furthermore, to ensure that we won't be visiting high correlated assets for a starting node in a node2vec with a walk length of grater than 1, we should also consider these properties in our transformation function:
\begin{itemize}
    \item 
    As the corresponding correlation of an edge approaches to 0, the edge's weight should approach infinity.
    \item
    As the corresponding correlation of an edge approaches to 1, the edge's weight should approach 0.
\end{itemize}


We used Hyperbolic Sine for our weight adjustment as it supported such properties. Then, The new redefinition of pairwise similarity between assets which was also used as the weight of the edges in our graph is calculated this way:

\begin{equation}
w_{ij} = \mid \coth(Correlation(i,j)) \mid -\coth(1)
\end{equation} 
As our graph is built, the next step is to run node2vec on our graph, for each node multiple random walks are executed based on the weights of its edges, that is in each step, the algorithm visits the neighbour $j$ of a starting node with a probability of $ \frac{w_{j}}{\sum_{i=1}^{n} w_{i}}$, where $w_j$ is the weight of the edge between the starting node and neighbour $j$, and the algorithm iterates over the graph in this manner $l$ times for each execution, where $l$ is the walk-length of the algorithm. In the end, a new pair-wise distance representation is created based on the nodes that have been visited during the execution of the algorithm for each starting node. Since we built the graph in a way that the edges with their corresponding nodes being uncorrelated, have a greater weight, we will visit uncorrelated nodes for each node after this algorithm.

We will then use soft k-means clustering on the newly created representation of our graph, and since our representation of the graph is produced so that the uncorrelated assets are closer to each other, we will reach clusters of rather uncorrelated assets which can be interpreted as selected assets for our diversified portfolio.



==> main/include/RelatedWorks-2.tex <==
\subsection{Related works}

After the initial widespread success of Markowitz's technique, lots of other approaches emerged in this area to enhance portfolio construction by modifying elements of the Markowitz technique or utilizing different approaches. Some attempts tried to improve the covariance estimation mechanism. \cite{ledoit2004well}\cite{wong2003efficient} Using graphs to model interactions between stocks is another approach. Mantegna (1998) was one of the first works that used graphs to suggest a portfolio. By finding an MST of the weighted graph, the method could find the hierarchical structure between stocks. Moreover, other combinatorial optimization methods are used to identify portfolios, as in \cite{boginski2014network}, which finding relaxed cliques in the network helps to identify similar stocks.

Machine learning techniques have also found their way in financial studies. In \cite{de2016building} authors use a hierarchical clustering approach to cluster stocks based on distances of their corresponding rows in the covariance matrix. Also, \cite{kumari2019mean} uses a k-means clustering approach to identify stock groups with the same characteristics.

Due to recent advances in deep learning methods, methods that try to use deep embeddings for stocks are also developed. For instance, \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method is able to identify groups of stocks that had similar price behavior as well as similar news. On
the other hand, \cite{hu2018deep} uses candlestick images and image neural network architectures to reach a proper representation for each stock.

While these representation learning methods use text and image data, to the best of our knowledge, no previous method uses the graph of relationships between stocks to derive embeddings for stocks.



==> main/include/RelatedWorks-3.tex <==
\subsection{Related works}

% Over the course of time, lots of different techniques and approaches formed to address the issue of portfolio optimization. One of the first and most famous theories was Markowitz’s Portfolio Theory [cite, 1952]. In his study, he utilized the covariance matrix of the financial assets to define the problem as a quadratic programming problem. The success of Markowitz’s theory embarked on the creation of many other methods in this field, and in fact most of portfolio construction and optimization methods have used the core idea of Markowitz’s theory, which is tha the lower the correlation of a portfolio's assets, the lower the risk of that portfolio. To point out a few successful portfolio construction methods based on Markowitz modern portfolio theory, we can name CLA [2013, cite] and MVO [cite]. There are also some other well-known approaches that are based on computational algorithms such as clustering, including HRP [cite], HERC [cite], and NCO [cite]. MANTANGE?

% There are variety of machine learning methods used for constructing portfolios. Some methods leverage optimization methods to overcome computational and estimation problems of portfolio optimization methods. \cite{still2010regularizing} uses a regularization method to construct weights that are stable and robust to fluctuations. \cite{perrin2020machine} investigates optimization methods to find a method that could be practically used for real-world problems with lots of assets. Some other studies, use prediction models to first predict each assets future dynamics and then use the predictions to find optimal assets. \cite{ta2018prediction}, \cite{chen2021mean}, \cite{ma2021portfolio} investigate a range of machine learning methods from simpler methods (Linear Regression \& Support Vector Regression) to more complex methods (XGBoost \& LSTMs). RL methods have also been studied, in which an agent learns how to construct appropriate portfolios by behaving in the environment \cite{yu2019model}.

After the initial widespread success of Markowitz’s technique, lots of other approaches emerged in this area to enhance portfolio construction by modifying elements of the Markowitz technique or utilizing different strategies. Some attempts tried to improve the covariance estimation mechanism \cite{ledoit2004well, wong2003efficient, ledoit2004well}. Other methods have considered higher-order moments to capture the relationships between assets better \cite{maringer2009global, khan2020sustainable}.

Instead of improving portfolio optimization methods directly, some methods approached the problem by first selecting a subset of assets and then weighting them to construct the portfolio. Mantegna \cite{mantegna99paper} was one of the works that did so by using graphs to suggest a subset of assets. By finding an MST of the weighted graph, the method could find the hierarchical structure between stocks. Moreover, other combinatorial optimization methods on graphs are used to identify portfolios, as in Boginski et al. \cite{boginski2014network}, in which finding relaxed cliques in the network helps identify similar stocks. Clustering techniques have also found their way into financial studies. In De Prado \cite{de2016building}, authors use a hierarchical clustering approach to cluster stocks based on distances of their corresponding rows in the covariance matrix. Also, Kumari et al. \cite{kumari2019mean} uses a k-means clustering approach to identify stock groups with the same characteristics.


Recently, machine learning methods have found their ways in financial market studies \cite{henrique2019literature}. Portfolio optimization was not an exception for this trend. Some methods in this area leverage optimization methods to overcome computational and estimation problems of portfolio optimization methods. \cite{still2010regularizing} uses a regularization method to construct weights that are stable and robust to fluctuations. \cite{perrin2020machine} investigates optimization methods to find a method that could be practically used for real-world problems with lots of assets. Some other studies use prediction models first to predict each asset's future dynamics and then use the predictions to find optimal assets. \cite{ta2018prediction, chen2021mean, ma2021portfolio} investigate a range of machine learning methods from simpler methods (Linear Regression \& Support Vector Regression) to more complex methods (XGBoost \& LSTMs \footnote{Long Short-Term Memory}). Reinforcement Learning (RL) methods have also been studied, in which an agent learns how to construct appropriate portfolios by behaving in the environment \cite{yu2019model}.

Due to the recent advances in deep learning methods, methods that try to use deep embeddings for stocks are also developed. For instance, Du \& Tanaka-Ishii \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method can identify groups of stocks that had similar price behavior as well as similar news. On the other hand, Hu et al. \cite{hu2018deep} uses candlestick images and image neural network architectures to reach a proper representation for each stock.

While these representation learning methods use text and image data, to the best of our knowledge, no previous method uses the graph of relationships between stocks to derive embeddings for stocks.



==> main/include/RelatedWorks.tex <==
\subsection{Related works}
% \begin{itemize}
%     \item The survey on portfolio selection.
%     \item The most basic available solutions
%     \item HRP, CLA
%     \item Graph-based solutions with the MST approach
%     \item Representation learning on candle images
% \end{itemize}
While Markowitz’s technique for portfolio optimization was a breakthrough method in financial asset management, its shortcomings are also well studied. The original intuition was to use the covariance matrix as an estimate for the connection between portfolios, to help invest in a diverse set of stocks that are their future is uncorrelated. However, major problems with this is method are investigated: (i) studies have shown that these estimations may not be accurate\cite{green1992will}\cite{ledoit2003improved}, and for having an appropriate estimate, the length of the historical data should grow as the number of stocks in interest grows. This issue will cause that in most real setups, this length should be as long as 3-4 years that is a long period and could not represent the recent relationships between stocks. \cite{chamberlain1982arbitrage}\cite{de2016building} (ii) output investment fractions are not stable, i.e., with introducing a small amount of noise to the data, the result could vary significantly.

To address these issues, lots of different approaches emerged in this area. Some attempts tried to improve the covariance estimation mechanism. \cite{ledoit2004well}\cite{wong2003efficient} Using graphs to model interactions between stocks is another approach. Mantegna (1998) was one of the first works that used graphs to suggest a portfolio. By finding an MST of the weighted graph, the method could find the hierarchical structure between stocks. Moreover, other combinatorial optimization methods are used to identify portfolios, as in \cite{boginski2014network}, which finding relaxed cliques in the network helps to identify similar stocks.

Machine learning techniques have also found their way in financial studies. In \cite{de2016building} authors use a hierarchical clustering approach to cluster stocks based on distances of their corresponding rows in the covariance matrix. Also, \cite{kumari2019mean} uses a k-means clustering approach to identify stock groups with the same characteristics.

Due to recent advances in deep learning methods, methods that try to use deep embeddings for stocks are also developed. For instance, \cite{du2020stock} uses text data like news articles related to each stock to design an embedding for stocks, then using clustering in the embedding space, the method is able to identify groups of stocks that had similar price behavior as well as similar news. On the other hand, \cite{hu2018deep} uses candlestick images and image neural network architectures to reach a proper representation for each stock. While these representation learning methods use text & image data, to the best of our knowledge, no previous method uses the graph of relationships between stocks to derive embeddings for stocks. To use machine learning and deep learning methods on graph structured data we have to first embed the graph or its nodes in a vector space. This task is well addressed in literature as representation learning for graphs which is to find an appropriate way to represent graph elements to best preserve the properties and relations of nodes that are required for solving the problem. There are different types of methods being used. Some of them use discrete metrics to define the similarity between nodes like the number of common neighbors \cite{ahmed2013distributed}\cite{cao2015grarep}. Others use random walks and the probability of observing one node while starting from another node as the similarity of the two nodes \cite{perozzi2014deepwalk}\cite{grover2016node2vec}. These two methods are unsupervised and don't require any labels on data. However, in case we have some labeled data we can use other methods that can use the labels in finding good representations. These methods also can better use other graph features. \cite{kipf2016semi}\cite{hamilton2017inductive}. Since our data is unlabeled and our initial metric (corrolation) was not discrete, we chose to use node2vec to apply it on the correlation graph of the stocks that we constructed, to reach a new similarity metric so that ultimately we can select a set of stocks which gives us a diversified portfolio.


==> main/include/Results.tex <==
\section{Results}
% \begin{itemize}
%     \item values of them?
%     \item K/N portfolio $->$ methods that construct small baskets, heuristics
%     \item S&P, NYSE, ...
%     \item Sharpe, risk, return.
%     \item Efficient frontier.

%     \item Discuss how changes in hyperparameters affect the results.
% \end{itemize}

% To evaluate the [RPS+optimization] model, we tested the results against various portfolio optimization algorithms. Since RPS is a portfolio selection algorithm, it can be combined with a generic type of optimization methods to enhance the performance of that particular algorithm. For this purpose, we used MVO[cite], CLA[cite], HRP\cite{de2016building}, and HERC[cite] to show RPS+optimization algorithm performs better than the algorithms themselves, without a selection method. These results show that a pre-selection of the portfolio is a dominant strategy to using the optimization algorithms alone, and furthermore, we show that our method performs better than other selection+optimization methods, such as random selection. [and simulated annealing?]
% For evaluating the created portfolios, we used efficient frontier and several financial criteria.
% [discussion]
% \begin{itemize}
% \item Sharpe Ratio:

% \begin{equation}
%     Sharpe\ Ratio = \frac{R_{p} - r_{f}}{\sigma_{p}}
% \end{equation}

% Where $R_{p}$ is return of the portfolio, $r_{f}$ is the risk free rate of return, and $\sigma{p}$ is the standard deviation of portfolio.

% \item Information Ratio:

% \begin{equation}
%  Information\ Ratio = \frac{R_{p} - R_{b}}{\sigma_{R_{p} - r_{b}}}     
% \end{equation}

% Where $R_{p}$ is return of the portfolio, $R_{b}$ is return of the benchmark, and $\sigma_{R_{p} - r_{b}}$ is the standard deviation of the excess return.

% \item
% M2 Measure (Modigliani):
% \begin{equation}
%  M2\ Measure = SR * \sigma_{b} + r_{f}   
% \end{equation}
% Where $SR$ is the Sharpe Ratio, $r_{f}$ is the risk free rate of return, and $\sigma_{b}$ is the standard deviation of benchmark.

% \end{itemize}
% [the above criteria are correlated somehow]

% To evaluate the [RPS+optimization] model, we have chosen the S&P dataset for training. We first trained the model on [folan] timeframe to attain the optimal selection. Then, we weighted the selections using the algorithms explained above and sorted the training results according to the criteria to achieve the best-selected portfolios. After this training phase, we used the exact weights to evaluate the portfolios in the next [timeframe].


% Also, table [number] shows the evaluation of methods using the mentioned criteria.

% [table]

% As it can be seen, we can enhance every optimization algorithm using pre-selection with the RPS model.

% RPS+OA vs. Random Pre-Selection+OA
% To show that the selected portfolios by the RPS method are solid selections, we evaluate the previous measurements for randomly selected portfolios. As a random portfolio has access to the whole efficient frontier area, a sufficient subset of random portfolios can sample the entire area, and thus, it would contain top portfolio selections.

% According to Figure \ref{fig:our_selection}, we can see that RPS+each optimization performs better than top random selections with the same optimization.


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{images/contribution-1-with-legend-all-dot.png}
    \caption{The efficient-frontier plot for the top 6 portfolios of the training set for RPS+optimization versus the algorithms without any selection phase.}
    \label{fig:our_selection}
\end{figure}

The data-set that we chose as a benchmark for our empirical results was S\&P 500, we used [timeframe] for training and [timeframe] as the testing period. Every weighted portfolio during the training period was evaluated with multiple financial ratios and the best performing portfolios were used in the following test timeframe.
The financial ratios which we used to evaluate the portfolios were as following:

\begin{itemize}
\item Sharpe Ratio:

\begin{equation}
    Sharpe\ Ratio = \frac{R_{p} - r_{f}}{\sigma_{p}}
\end{equation}

Where $R_{p}$ is return of the portfolio, $r_{f}$ is the risk free rate of return, and $\sigma{p}$ is the standard deviation of portfolio.

\item Information Ratio:

\begin{equation}
 Information\ Ratio = \frac{R_{p} - R_{b}}{\sigma_{R_{p} - r_{b}}}     
\end{equation}

Where $R_{p}$ is return of the portfolio, $R_{b}$ is return of the benchmark, and $\sigma_{R_{p} - r_{b}}$ is the standard deviation of the excess return.

\item
M2 Measure (Modigliani):
\begin{equation}
 M2\ Measure = SR * \sigma_{b} + r_{f}   
\end{equation}
Where $SR$ is the Sharpe Ratio, $r_{f}$ is the risk free rate of return, and $\sigma_{b}$ is the standard deviation of benchmark.

\end{itemize}

We have done two sets of experiments which we will present.

\begin{table*}[!h]
\centering
\caption{Portfolios built with different settings can be seen here with their respective performance measurements. It can be seen that for each different portfolio optimization algorithm, applying RPS as an asset selection method improves the performances for the portfolio.}
\label{tab:evaluations}
\begin{tabular}{l|c|c|c|}
\cline{2-4}
                                              & \multicolumn{1}{l|}{Sharpe Ratio} & \multicolumn{1}{l|}{Information Ratio} & \multicolumn{1}{l|}{Modiliani Risk Adjusted Performance} \\ \hline
\multicolumn{1}{|l|}{\textbf{RPS+MVO}}        & 5.785917                          & 4.151003                               & 1.345936                               \\ \hline
\multicolumn{1}{|l|}{Best Random Subset+MVO}  & 5.014807                          & 3.459654                               & 1.167744                               \\ \hline
\multicolumn{1}{|l|}{MVO}                     &            -                       &                                        &                                        \\ \hline
\multicolumn{1}{|l|}{\textbf{RPS+HRP}}        & 4.507241                          & 2.851294                               & 1.050454                               \\ \hline
\multicolumn{1}{|l|}{Best Random Subset+HRP}  & 3.607982                          & 3.826712                               & 0.842649                               \\ \hline
\multicolumn{1}{|l|}{HRP} &     -1.276275               &                                   &                                                                                \\ \hline
\multicolumn{1}{|l|}{\textbf{RPS+HERC}}       & 4.458710                          & 2.703551                               & 1.039239                               \\ \hline
\multicolumn{1}{|l|}{Best Random Subset+HERC} & 2.664600                          & 1.970464                               & 0.624648                               \\ \hline
\multicolumn{1}{|l|}{HERC}  &        -1.294033           &                                   &                                                                                \\ \hline
\multicolumn{1}{|l|}{\textbf{RPS+CLA}}        & 6.734292                          & 4.480901                               & 1.565091                               \\ \hline
\multicolumn{1}{|l|}{Best Random Subset+CLA}  & 8.920160                          & 4.928809                               & 2.070211                               \\ \hline
\multicolumn{1}{|l|}{CLA}    &    -1.924916             &                                   &                                                                                \\ \hline
\end{tabular}
\end{table*}

\subsection{RPS+POA vs. POA}

Since RPS is a portfolio selection algorithm, it can be combined with a generic type of Portfolio Optimization Method to enhance the performance of that algorithm. To evaluate the RPS method, we used selected subsets of assets calculated by RPS, and optimized the subsets with various optimization methods such as CLA[cite], HRP\cite{de2016building}, and HERC[cite], thus reaching a weighted portfolio which we will call RPS+POA (Representation Portfolio Selection + Portfolio Optimization Algorithm). Then we compared performance of the RPS+POA portfolio with the portfolio built with the corresponding Portfolio Optimization Algorithm, which is shown in Figure \ref{fig:our_selection}.
As it is indicated in the the figure, RPS enhances all of the mentioned portfolio optimization algorithms. The numerical comparisons are shown in Table \ref{tab:evaluations}.

Furthermore there are portfolio optimization algorithms which can not be used on a whole benchmark of assets and they need to have a subset of assets so that they can operate functionally. For instance, MVO[cite] might not converge when given a big benchmark of assets. Such methods benefit from the asset selection of RPS.

\subsection{RPS+POA vs. Random-Selected-Assets+POA}

To  show  that  the  selected  portfolios  by  the  RPS  method are  solid  selections,  we  evaluate  the  previous  measurements for  randomly  selected  portfolios.  As  a  random  portfolio  has access  to  the  whole  efficient  frontier  area,  a  sufficient  subset of  random  portfolios  can  sample  the  entire  area,  and  thus,  it would contain top portfolio selections. We generated more than 13k random portfolios, which took the same time as RPS to train on the market data and calculate its heuristically optimal subset of assets. Figure 3 shows the comparison between performance of RPS+POA portfolios and Random-Selected-Assets+POA portfolios on test data. Since only the top random portfolios of the train data will be chosen as potential portfolios for the test data, only the top 5(?) portfolios in terms of Sharpe Ratio out of all the generated Random-Selected-Assets have been shown on this figure.



% [explain the extra column, the betterness-average]
% [RPS+OA vs. other pre-selections?+OA]


%We chose S&P500 stocks for practical demonstration of our portfolio selection algorithm, we call our method RPS (Representation Portfolio Selection). To show how RPS and pre-selection of assets improves portfolio optimization methods, we built several portfolios using different portfolio optimization algorithms with 3 different variations, with no asset selection beforehand, with pre-selection using random assets, and with RPS asset selection method which we proposed in our papaer. The results can be seen in table 1, where it shows that that for each portfolio optimization method, the RPS variant outperforms the others.




==> main/include/Results2.tex <==
\section{Results}

\subsection{Datasets}

To test our method in an empirical experiment, we chose three datasets from three different stock market indices in different timeframes.
Descriptions of the datasets that we used can be observed in Table \ref{tab:datasets}.
The S\&P 500 data is available in daily resolution
The Nikkei 225 and S\&P 100 datasets were obtained from Indextrack datasets \cite{BEASLEY2003621}. The prices in this dataset are indexed from 0 to 291, which are the weekly prices between March 1992 to September 1997, and the train and test ranges are expressed as an index value in Table \ref{tab:datasets}.

\begin{table}[]
    \centering
   \caption{Datasets Information}
    \begin{tabularx}{0.45\textwidth}{|*{4}{c}}
    \hline
    
    \multicolumn{1}{|p{1.86cm}|}{Index} & \multicolumn{1}{p{1.86cm}|}{Asset Count} & \multicolumn{1}{p{1.86cm}|}{Train Range} & \multicolumn{1}{p{1.86cm}|}{Test Range} \\ \hline
    
    \multicolumn{1}{|p{1.86cm}|}{S\&P 500} & \multicolumn{1}{p{1.86cm}|}{465} & \multicolumn{1}{p{1.86cm}|}{2019-04-01 to 2019-08-01} & \multicolumn{1}{p{1.86cm}|}{2019-08-02 to 2019-09-01} \\ \hline
    
    \multicolumn{1}{|p{1.86cm}|}{Nikkei 225} & \multicolumn{1}{p{1.86cm}|}{225} & \multicolumn{1}{p{1.86cm}|}{0 to 200} & \multicolumn{1}{p{1.86cm}|}{201 to 290} \\ \hline
    
    \multicolumn{1}{|p{1.86cm}|}{S\&P 100} & \multicolumn{1}{p{1.86cm}|}{98} & \multicolumn{1}{p{1.86cm}|}{0 to 200} & \multicolumn{1}{p{1.86cm}|}{201 to 290} \\ \hline
    
    \end{tabularx}
    \label{tab:datasets}
\end{table}

\subsection{Metrics}

We used two approaches to evaluate the performance of the algorithms used in our paper. We measured the future performances of their output portfolios using several financial metrics and assessed their stability both in time and against noise via computational methods.

The financial ratios which we used to evaluate the future performance of portfolios were as following:

\begin{itemize}

\item Correlation: Since our method's primary focus was to minimize the correlation between different assets' price values, we must evaluate how minimization of correlation in train data relates to the correlation of portfolios in the test data. All of the other measures are a byproduct of this value.

\item Return: The return of the portfolios was evaluated in the test range.

\item Risk: The risk of the portfolios is defined as the standard deviation of the asset returns in a given time range.

\item Sharpe Ratio:
\begin{equation}
    Sharpe\ Ratio = \frac{R_{p} - r_{f}}{\sigma_{p}}
\end{equation}

Where $R_{p}$ is the return of the portfolio, $r_{f}$ is the risk-free rate of return, and $\sigma{p}$ is the standard deviation of the portfolio.

\item
Information Ratio:
\begin{equation}
 Information\ Ratio = \frac{R_{p} - R_{b}}{\sigma_{R_{p} - r_{b}}}     
\end{equation}

Where $R_{p}$ is return of the portfolio, $R_{b}$ is return of the benchmark, and $\sigma_{R_{p} - r_{b}}$ is the standard deviation of the excess return.

\item
M2 Measure (Modigliani):
\begin{equation}
 M2\ Measure = SR * \sigma_{b} + r_{f}   
\end{equation}
Where $SR$ is the Sharpe Ratio, $r_{f}$ is the risk-free rate of return, and $\sigma_{b}$ is the standard deviation of the benchmark.

\end{itemize}

To evaluate the stability of the algorithms, we took another approach.

\newtheorem{dfn}{Definition}
\begin{dfn}
Suppose that the training phase of an algorithm has resulted in $k_1$ different portfolios, where each is a set of assets. If the model is trained again under different circumstances, the result of the train would be $k_2$ portfolios. A stability matrix ($SM$) is defined as a $k_1 \times k_2$ matrix where $SM_{ij}$ is the similarity value between portfolio $i$ of the first train phase and portfolio $j$ of the second train phase.
\end{dfn}

The similarity metric we used in this paper was Jaccard Similarity measures, which is defined as below between set $A$ and set $B$:

\begin{equation}
    JaccardSim(A, B) = \frac{|A \cap B|}{|A \cup B|}
\end{equation}

Where $|S|$ is the size of set $S$. We use a matrix instead of a list because we cannot determine an injective function between two phases of training, and therefore no direct mapping exists between two sets of portfolios. After forming the stability matrix, we can extract different measures from it. First of all, we calculate the maximum similarity value for each portfolio to find a mapping between phases. One problem in this process is that the count of portfolios can vary between phases. For example, since the Louvain clustering algorithm does not provide input for several clusters, the output cluster count might differ in different training sets. Furthermore, some of the weighting algorithms might not reach a conversion point for a specific portfolio, and therefore the subset would not be present in the training process results. As a result of this problem, the column-wise maximum of the matrix is not necessarily equal to the row-wise maximum. We combine the row-wise and the column-wise maximums before any further inspections to create a symmetric measure from the similarity matrix.

After taking the maximums, we use the average of maximums to compute the stability of the algorithm. As mentioned before, we also use two different stability tests:

\begin{itemize}
    \item Noise Stability: The stability of the method if a minuscule amount of Gaussian noise is applied to the correlation matrix of the assets.
    \item Time Stability: The method's stability if the time range of the training dataset is shifted for a small amount.
\end{itemize}

Note that these stability functions cannot be applied to Random and Simulated Annealing selection methods since they are statistical approaches for the optimization problem and unstable. No two consecutive runs with similar conditions would result in the same portfolio using these methods.

\subsection{Experiments}

\paragraph{Future Performance} To measure the performance of RPS for each of the datasets that we had, we constructed several portfolios using different methods and compared their performances via the metrics that we described above. Firstly, we built a set of portfolios with a two-phased approach that used RPS for their asset selection in their first phase, and then used one of the portfolio optimization methods CLA \cite{niedermayer2010CLA}, MVO \cite{erlich2010MVO}, or HRP \cite{pfitzinger2019HRP}. Then we created a set of other portfolios using our benchmark methods. Three out of four of these methods, Mantegna (MTN), Random (RND), and Graph Splex (SPX), can be used in a two-phased fashion like ours. After computing the subsets, we used the same portfolio optimization methods mentioned above. The Simulated Annealing (SA) method is a one-phased method, and the result of its training contains the weights and portfolios. Furthermore, RPS and MTN methods result in multiple portfolios. We ran RND and SA multiple times to compare all of the benchmarks, but the SPX approach outputs a consistent result for a given market. Lastly, we could not run the SPX method on Nikkei 225 and S\&P 500 datasets since it did not converge on our systems in a bounded time.

The top 10 portfolios in the training range of each method were then picked, and their performances were evaluated in the test range. Portfolios were sorted using Sharpe value to maximize the return while minimizing the risk. The risk-return graph depicting the discussed portfolios can be observed in Figure \ref{fig:our_selection}.

\begin{figure}[!ht]
    \label{fig:our_selection}
    \centering
    \includegraphics[width=0.46\textwidth]{main/images/risk_return_idx4.png}
    \includegraphics[width=0.46\textwidth]{main/images/risk_return_idx5.png}
    \includegraphics[width=0.46\textwidth]{main/images/risk_return_sp500.png}
    \caption{The efficient-frontier plot for the top 10 portfolios of the training set for RPS+optimization versus benchmark algorithms.}
\end{figure}

Moreover, the best value of future metrics for each of the methods are available in Tables \ref{tab:sp500fp}, \ref{tab:nikkeifp}, and \ref{tab:sp100fp}.

\begin{table*}[!t]
  \centering
  \caption{Future Performance Measures for S\&P 500 Dataset}
  \begin{tabular}{ccccccc}
    \hline
    Method & Correlation & Return & Risk & Sharpe Ratio & Information Ratio & M2 \\
    \hline
    Vanilla CLA & 0.162075 & 0.027747 & 0.114838 & 0.164118 & 0.242098 & 0.027636  \\
    RPS+CLA & 0.138791 & \textbf{1.110586} & 0.369897 & 3.435445 & \textbf{4.721627} & 0.817560 \\
    MTN+CLA & 0.196280 & 1.094718 & 0.369051 & \textbf{4.948828} & 4.654215 & \textbf{1.173791} \\
    RND+CLA & 0.171342 & 0.267575 & 0.535209 & 1.031657 & 1.140248 & 0.251739 \\
    \hline
    Vanilla HRP & 0.162075 & 0.011727 & \textbf{0.095295} & 0.216459 & 0.103681 & 0.015811  \\
    RPS+HRP & \textbf{0.008178} & 0.535214 & 0.269456 & 2.153089 & 2.277263 & 0.515710 \\
    MTN+HRP & 0.196280 & 0.541221 & 0.270475 & 3.698830 & 2.302783 & 0.879557  \\
    RND+HRP & 0.191148 & 0.166312 & 0.291356 & 0.773329 & 0.710050 & 0.190932 \\
    \hline
    Vanilla MVO & 0.162075 & 0.027747 & 0.114838 & 0.164118 & 0.242098 & 0.027636  \\
    RPS+MVO & 0.138791 & 0.932556 & 0.285581 & 4.163090 & 3.965298 & 0.988838 \\
    MTN+MVO & 0.235134 & 0.557674 & 0.215301 & 3.736161 & 2.372682 & 0.888345 \\
    RND+MVO & 0.174462 & 0.165436 & 0.262077 & 0.597288 & 0.706327 & 0.149494 \\
    \hline
    SA & 0.167465 & 0.273648 & 0.210593 & 1.117717 & 1.166047 & 0.271996  \\ \hline
  \end{tabular}
  \label{tab:sp500fp}
\end{table*}

\begin{table*}[!t]
  \centering
  \caption{Future Performance Measures for Nikkei 225 Dataset}
  \begin{tabular}{ccccccc}
    \hline
    Method & Correlation & Return & Risk & Sharpe Ratio & Information Ratio & M2 \\
    \hline
    Vanilla CLA & 0.450845 & 0.143052 & 0.436134 & 0.261482 & 0.278425 & 0.142717  \\
    RPS+CLA & \textbf{0.094671} & \textbf{1.991665} & 0.387936 & 3.818792 & \textbf{4.599676} & 1.665158 \\
    MTN+CLA & 0.210820 & 0.395800 & 0.403417 & 0.790543 & 0.920129 & 0.351768 \\
    RND+CLA & 0.189425 & 0.962127 & 0.398781 & 2.390352 & 2.225895 & 1.045625 \\
    \hline
    Vanilla HRP & 0.450845 & 0.042383 & 0.422741 & 0.069599 & 0.081713 & 0.044518  \\
    RPS+HRP & 0.176072 & 0.165529 & 0.403649 & 0.385897 & 0.389200 & 0.176268 \\
    MTN+HRP & 0.210820 & 0.946481 & 0.354701 & 2.427145 & 2.189820 & 1.061583 \\
    RND+HRP & 0.265348 & -0.411154 & 0.405019 & -1.037120 & -0.940445 & -0.440912 \\
    \hline
    Vanilla MVO & 0.450845 & 0.143052 & 0.436134 & 0.261482 & 0.278425 & 0.142717  \\
    RPS+MVO & \textbf{0.094671} & 1.978367 & 0.400116 & \textbf{3.826142} & 4.569014 & \textbf{1.668345} \\
    MTN+MVO & 0.210820 & 0.594692 & \textbf{0.352680} & 1.520505 & 1.378710 & 0.668362 \\
    RND+MVO & 0.105741 & -0.315837 & 0.374047 & -0.868171 & -0.720674 & -0.367636 \\
    \hline
    SA & 0.558230 & -0.937416 & 0.420207 & -2.070724 & -2.153834 & -0.889199 \\
    \hline
  \end{tabular}
  \label{tab:nikkeifp}
\end{table*}

\begin{table*}[!t]
  \centering
  \caption{Future Performance Measures for S\&P 100 Dataset}
  \begin{tabular}{ccccccc}
    \hline
    Method & Correlation & Return & Risk & Sharpe Ratio & Information Ratio & M2 \\
    \hline
    Vanilla CLA & 0.418337 & 1.269428 & 0.198022 & 4.348930 & 4.385291 & 1.262862 \\
    RPS+CLA & 0.177503 & 2.783124 & 0.481028 & 4.457300 & 9.635014 & 1.294110 \\
    MTN+CLA & 0.155783 & 2.630134 & 0.402634 & 4.461950 & 9.104422 & 1.295450 \\
    SPX+CLA & 0.870104 & 2.461136 & 0.571726 & 4.289180 & 8.518312 & 1.245634 \\
    RND+CLA & 0.208234 & \textbf{3.696725} & 0.320223 & \textbf{5.226347} & \textbf{12.803521} & \textbf{1.515855} \\
    \hline
    Vanilla HRP & 0.418337 & 1.278512 & 0.195795 & 4.449693 & 4.416796 & 1.291916 \\
    RPS+HRP & 0.255930 & 1.473516 & 0.257972 & 3.724968 & 5.093098 & 1.082950 \\
    MTN+HRP & 0.155783 & 2.100452 & 0.298370 & 4.351074 & 7.267409 & 1.263480 \\
    SPX+HRP & 0.870104 & 2.585765 & 0.627108 & 4.109122 & 8.950544 & 1.193717 \\
    RND+HRP & 0.206733 & 1.548159 & \textbf{0.252117} & 4.243590 & 5.351972 & 1.232489 \\
    \hline
    Vanilla MVO & 0.418337 & 1.269428 & 0.198022 & 4.348930 & 4.385291 & 1.262862 \\
    RPS+MVO & 0.177503 & 2.790539 & 0.481578 & 4.476027 & 9.660732 & 1.299509 \\
    MTN+MVO & 0.339761 & 1.914374 & 0.303960 & 4.823667 & 6.622061 & 1.399747 \\
    SPX+MVO & 0.870104 & 2.461136 & 0.571726 & 4.289180 & 8.518312 & 1.245634 \\
    RND+MVO & \textbf{0.043606} & 1.634323 & 0.306306 & 4.889193 & 5.650800 & 1.418641 \\
    \hline
    SA & 0.217874 & 1.759462 & 0.326334 & 4.851917 & 6.084802 & 1.407893 \\
    \hline
  \end{tabular}
  \label{tab:sp100fp}
\end{table*}

It can be seen in these tables that in S\&P 500 and Nikkei 225, RPS has reached the best possible return among other methods and also the best correlation value. It can be seen that selection in all of the instances caused the correlation value to decrease from the original correlation of the assets. However, the results of performances are pretty different in S\&P 100 database. It is consistent with the notion that a random selection phase can lead to relatively high-performance portfolios since it can reach any point in the space of portfolios. The relative lousy performance of all other algorithms can be explained by looking at the correlation of all the assets in the dataset. The overall average correlation between assets of S\&P 100 is equal to 0.418337. Since the market assets are highly correlated, it becomes harder for the selection algorithms to find a highly uncorrelated subset, and therefore, most of the portfolios would move in the direction of the general trend. Both good performance of selection algorithms and bad performance of random selection in Nikkei 255 and bad performance of selection algorithms and good performance of random selection in S\&P 100 can be explained using this argument. Moreover, we can inspect the return of all portfolios in the markets in Figure \ref{fig:return_dist}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{main/images/returns_dist_idx4.png}
    \includegraphics[width=0.47\textwidth]{main/images/returns_dist_idx5.png}
    \includegraphics[width=0.47\textwidth]{main/images/returns_dist_sp500.png}
    \caption{Return distribution}
    \label{fig:return_dist}
\end{figure}

It can be seen in Figure \ref{fig:return_dist} that RPS achieves a higher average return. In S\&P 100, few of the RND portfolios were able to reach a high return value, and also SPX achieves a higher average return, but as can be seen in the figure, RPS can obtain higher average performance.

\paragraph{Stability} The time and noise stability metrics are shown in table \ref{tab:ns} and \ref{tab:ts}. Gaussian noise with $\mu=0$ and $\sigma=0.01$ was applied to the market correlation matrix for noise stability. For time stability, the train time ranges were shifted to 20 data points for each dataset.

\begin{table}[!hbtp]
  \centering
  \caption{Noise Stability}
  \begin{tabular}{cccc}
    \hline
    Method & S\&P 100 & Nikkei 225 & S\&P 500 \\ \hline
    Mantegna & \textbf{0.528711} & \textbf{0.479277} & \textbf{0.427159} \\
    RPS & 0.460720 & 0.373794 & 0.085135 \\
    Splex & 0.000000 & - & - \\
    \hline
  \end{tabular}
  \label{tab:ns}
\end{table}

\begin{table}[!hbtp]
  \centering
  \caption{Time Stability}
  \begin{tabular}{cccc}
    \hline
    Method & S\&P 100 & Nikkei 225 & S\&P 500 \\ \hline
    Mantegna & 0.336598 & \textbf{0.360965} & \textbf{0.228190} \\
    RPS & \textbf{0.557390} & 0.231124 & 0.119387 \\
    Splex & 0.400000 & - & - \\
    \hline
  \end{tabular}
  \label{tab:ts}
\end{table}

In noise stability metrics, MTN was able to outperform RPS and SPX methods. However, the margin of superiority was not significant in the S\&P 100 dataset, resulting from the smaller size of the database and the lower number of options available in the selection phase. As the size of the dataset grows, stability drops for all of the methods.

\paragraph{RPS Clustering Method} Another issue to analyze is whether the clustering method (k-means or fuzzy c-means) affects outcoming portfolios or not. Figure \ref{fig:rps_cluster} depicts the risk-return relation for all different setups of RPS ran in the test range.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{main/images/rps_cluster_method.png}
    \caption{Risk-Return distribution of RPS on S\&P 500 dataset, separated by clustering method.}
    \label{fig:rps_cluster}
\end{figure}

As seen in this figure, there are no significant differences between the portfolios using these two clustering methods.

==> main/include/abstract.tex <==
% As a general rule, do not put math, special symbols or citations
% in the abstract
\begin{abstract}
Portfolio optimization is one of the essential fields of focus in finance. There has been an increasing demand for novel computational methods in this area to compute portfolios with better returns and lower risks in recent years. We present a novel computational method called Representation Portfolio Selection (RPS) by redefining the distance matrix of financial assets using Representation Learning and Clustering algorithms for portfolio selection to increase diversification. RPS proposes a heuristic for getting closer to the optimal subset of assets. Using empirical results in this paper, we demonstrate that widely used portfolio optimization algorithms, such as MVO, CLA, and HRP, can benefit from our asset subset selection.
\end{abstract}
